Chain-of-Layer: Iteratively Prompting Large Language Models for Taxonomy Induction from Limited Examples

Automatic taxonomy induction is crucial for web search, recommendation systems, and question answering. Manual curation of taxonomies is expensive in terms of human effort, making automatic taxonomy construction highly desirable. In this work, we introduce Chain-of-Layer which is an in-context learning framework designed to induct taxonomies from a given set of entities. Chain-of-Layer breaks down the task into selecting relevant candidate entities in each layer and gradually building the taxonomy from top to bottom. To minimize errors, we introduce the Ensemble-based Ranking Filter to reduce the hallucinated content generated at each iteration. Through extensive experiments, we demonstrate that Chain-of-Layer achieves state-of-the-art performance on four real-world benchmarks.

==> Figures/raw/CoL-Overview <==
<mxfile host="app.diagrams.net" modified="2024-02-06T09:21:48.886Z" agent="Mozilla/5.0 (Macintosh; Intel Mac OS X 10_15_7) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/121.0.0.0 Safari/537.36" etag="U-Fv49lB2wMMxp90T7NX" version="23.1.1" type="device">
  <diagram name="Page-1" id="Page-1">
    <mxGraphModel dx="2709" dy="284" grid="1" gridSize="10" guides="1" tooltips="1" connect="1" arrows="1" fold="1" page="1" pageScale="1" pageWidth="2184" pageHeight="863" math="1" shadow="0">
      <root>
        <mxCell id="0" />
        <mxCell id="1" parent="0" />
        <mxCell id="RbdjuNJBBSJslo0sPhe3-332" style="vsdxID=802;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;entryX=0.811;entryY=0.988;entryDx=0;entryDy=0;entryPerimeter=0;exitX=0.527;exitY=0.012;exitDx=0;exitDy=0;exitPerimeter=0;" edge="1" parent="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="808.38" y="542" as="sourcePoint" />
            <mxPoint x="808.38" y="505" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="5" style="vsdxID=228;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="372" y="99" width="529" height="490" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-330" style="vsdxID=802;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;entryX=0.811;entryY=0.988;entryDx=0;entryDy=0;entryPerimeter=0;exitX=0.527;exitY=0.012;exitDx=0;exitDy=0;exitPerimeter=0;" edge="1" parent="1" source="12">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="621" y="540" as="sourcePoint" />
            <mxPoint x="621" y="506" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-329" style="vsdxID=802;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.575;exitY=0.001;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.811;entryY=0.988;entryDx=0;entryDy=0;entryPerimeter=0;" edge="1" parent="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="469.4749999999999" y="542.042" as="sourcePoint" />
            <mxPoint x="470" y="506" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="11" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;geometry&lt;/font&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt; is a &amp;lt;mask&amp;gt;&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=179;fillColor=#e4ffff;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);dashed=1;strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="403" y="542" width="133" height="42" as="geometry" />
        </mxCell>
        <mxCell id="12" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;geometry&lt;/font&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt; is a type of &amp;lt;mask&amp;gt;&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=180;fillColor=#dae2f3;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);dashed=1;strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="551" y="542" width="133" height="42" as="geometry" />
        </mxCell>
        <mxCell id="13" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&amp;lt;mask&amp;gt; such as&lt;/font&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt; &lt;/font&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;geometry&lt;/font&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt; &#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=181;fillColor=#e2efd9;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);dashed=1;strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="742" y="542" width="133" height="42" as="geometry" />
        </mxCell>
        <mxCell id="14" value="&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;...&#xa;&lt;/font&gt;" style="verticalAlign=middle;align=center;vsdxID=182;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="699" y="557" width="30" height="11" as="geometry" />
        </mxCell>
        <mxCell id="16" value="&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;...&#xa;&lt;/font&gt;" style="verticalAlign=middle;align=center;vsdxID=184;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="698" y="456" width="30" height="11" as="geometry" />
        </mxCell>
        <mxCell id="17" style="vsdxID=185;fillColor=none;gradientColor=none;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="403" y="418" width="133" height="89" as="geometry" />
        </mxCell>
        <mxCell id="18" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;&amp;lt;mask&amp;gt;&#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=186;fillColor=#e4ffff;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="17" vertex="1">
          <mxGeometry width="90" height="22" as="geometry" />
        </mxCell>
        <mxCell id="19" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;R (S)&#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=187;fillColor=#e4ffff;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="17" vertex="1">
          <mxGeometry x="82" width="50" height="22" as="geometry" />
        </mxCell>
        <mxCell id="20" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;mathematic&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=188;fillColor=#e4ffff;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="17" vertex="1">
          <mxGeometry y="22" width="82" height="22" as="geometry" />
        </mxCell>
        <mxCell id="21" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;1 (1/1)&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=189;fillColor=#e4ffff;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="17" vertex="1">
          <mxGeometry x="82" y="22" width="50" height="22" as="geometry" />
        </mxCell>
        <mxCell id="22" style="vsdxID=190;fillColor=#e4ffff;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="17" vertex="1">
          <mxGeometry y="44" width="82" height="22" as="geometry" />
        </mxCell>
        <mxCell id="23" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;...&#xa;&lt;/font&gt;&lt;/p&gt;" style="text;vsdxID=190;fillColor=none;gradientColor=none;rotation=270.05;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;verticalAlign=middle;align=center;;html=1;" parent="22" vertex="1">
          <mxGeometry y="-0.21" width="82.55" height="22.21" as="geometry" />
        </mxCell>
        <mxCell id="24" style="vsdxID=191;fillColor=#e4ffff;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="17" vertex="1">
          <mxGeometry x="82" y="44" width="50" height="22" as="geometry" />
        </mxCell>
        <mxCell id="25" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;...&#xa;&lt;/font&gt;&lt;/p&gt;" style="text;vsdxID=191;fillColor=none;gradientColor=none;rotation=270.05;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;verticalAlign=middle;align=center;;html=1;" parent="24" vertex="1">
          <mxGeometry y="-0.21" width="50.68" height="22.21" as="geometry" />
        </mxCell>
        <mxCell id="26" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;physics&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=192;fillColor=#e4ffff;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="17" vertex="1">
          <mxGeometry y="66" width="82" height="22" as="geometry" />
        </mxCell>
        <mxCell id="27" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;5 (1/5)&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=193;fillColor=#e4ffff;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="17" vertex="1">
          <mxGeometry x="82" y="66" width="50" height="22" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-678" style="vsdxID=715;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="-1896" y="426" width="1237" height="240.5" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-354" value="" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#FFF4FE;strokeColor=#9673a6;labelBackgroundColor=#FFF4FE;" parent="1" vertex="1">
          <mxGeometry x="-1260" y="434.5" width="590" height="223.5" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-352" value="" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#dae8fc;strokeColor=#6c8ebf;" parent="1" vertex="1">
          <mxGeometry x="-1886.66" y="436.25" width="586.66" height="223.5" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-315" value="&lt;font style=&quot;font-size:33px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;Overall Pipeline&#xa;&lt;/b&gt;&lt;/font&gt;" style="verticalAlign=top;align=center;vsdxID=852;fillColor=#f2f2f2;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=none;strokeWidth=2;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="-1898" y="161.5" width="1238" height="245" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-413" style="vsdxID=715;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="-1600" y="216.5" width="537" height="173.5" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-414" style="vsdxID=717;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="-1560" y="264.5" width="150" height="111" as="geometry" />
        </mxCell>
        <mxCell id="125" style="vsdxID=479;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);dashed=1;strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="384" y="137" width="238" height="117" as="geometry" />
        </mxCell>
        <mxCell id="9" value="&lt;p style=&quot;align:left;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:top;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:19px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt; &lt;/b&gt;&lt;/font&gt;&lt;font style=&quot;font-size:25px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;Select&lt;/b&gt;&lt;/font&gt;&lt;font style=&quot;font-size:25px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt; entity list&lt;/b&gt;&lt;/font&gt;&lt;font style=&quot;font-size:25px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;&#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;&lt;p style=&quot;align:left;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:top;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;Prompt:&lt;/b&gt;&lt;/font&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;i&gt; &lt;/i&gt;&lt;/font&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;i&gt;Then, let&amp;prime;s find all the k-level entities from the remaining entity list.&lt;/i&gt;&lt;/font&gt;&lt;font style=&quot;font-size:19px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;i&gt;&#xa;&lt;/i&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=top;align=left;vsdxID=175;fillColor=#deebf6;gradientColor=none;shape=stencil(rVLLDsIgEPwVsndaWh+tCeVfiNKWiKXZotW/l5ZY0YsmeiLMkplhdvjQyl6RwaE9qlEfXFuB7lqF2oHgtUXVoD13B8F76VrBT/aiyLWCjAG5TQeDVHCjuxndfYFK3BOc0KTcAkE/yFmyXkFgDU+LXZKXHqHyqgeK1kmnbVeBnxqJjaKehNZGNjM0jEr1yzUSftB5gSJ/1S7Wi3ZWQOSSst91n1QvZj6BUTLlM5ngLv7Iz/7ikCPdjCVsswiXObwt+g/7iIuQhkbV2phQvwmLG5fO3RR3);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="1343" y="472" width="243" height="117" as="geometry" />
        </mxCell>
        <mxCell id="75" style="vsdxID=409;fillColor=none;gradientColor=none;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="565" y="280" width="188" height="89" as="geometry" />
        </mxCell>
        <mxCell id="76" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;Rank&#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=213;fillColor=#fbe5d5;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="75" vertex="1">
          <mxGeometry width="53" height="22" as="geometry" />
        </mxCell>
        <mxCell id="77" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;Entity Candidates&#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=214;fillColor=#fbe5d5;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="75" vertex="1">
          <mxGeometry x="51" width="136" height="22" as="geometry" />
        </mxCell>
        <mxCell id="78" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:12px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;1&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=215;fillColor=#fbe5d5;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="75" vertex="1">
          <mxGeometry y="22" width="53" height="22" as="geometry" />
        </mxCell>
        <mxCell id="79" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;mathematic&lt;/font&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=216;fillColor=#fbe5d5;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#3955a3;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="75" vertex="1">
          <mxGeometry x="51" y="22" width="136" height="22" as="geometry" />
        </mxCell>
        <mxCell id="80" style="vsdxID=217;fillColor=#fbe5d5;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="75" vertex="1">
          <mxGeometry y="44" width="53" height="22" as="geometry" />
        </mxCell>
        <mxCell id="81" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;...&#xa;&lt;/font&gt;&lt;/p&gt;" style="text;vsdxID=217;fillColor=none;gradientColor=none;rotation=270.05;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;verticalAlign=middle;align=center;;html=1;" parent="80" vertex="1">
          <mxGeometry y="-0.21" width="53.83" height="22.21" as="geometry" />
        </mxCell>
        <mxCell id="82" style="vsdxID=218;fillColor=#fbe5d5;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="75" vertex="1">
          <mxGeometry x="51" y="44" width="136" height="22" as="geometry" />
        </mxCell>
        <mxCell id="83" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;...&#xa;&lt;/font&gt;&lt;/p&gt;" style="text;vsdxID=218;fillColor=none;gradientColor=none;rotation=270.05;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;verticalAlign=middle;align=center;;html=1;" parent="82" vertex="1">
          <mxGeometry y="-0.21" width="136.94" height="22.21" as="geometry" />
        </mxCell>
        <mxCell id="84" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;n&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=219;fillColor=#fbe5d5;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="75" vertex="1">
          <mxGeometry y="66" width="53" height="22" as="geometry" />
        </mxCell>
        <mxCell id="85" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;physics&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=220;fillColor=#fbe5d5;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="75" vertex="1">
          <mxGeometry x="51" y="66" width="136" height="22" as="geometry" />
        </mxCell>
        <mxCell id="86" style="vsdxID=221;fillColor=none;gradientColor=none;image;aspect=fixed;image=data:image/png,/9j/4AAQSkZJRgABAQAAAQABAAD/2wBDAAgGBgcGBQgHBwcJCQgKDBQNDAsLDBkSEw8UHRofHh0aHBwgJC4nICIsIxwcKDcpLDAxNDQ0Hyc5PTgyPC4zNDL/2wBDAQkJCQwLDBgNDRgyIRwhMjIyMjIyMjIyMjIyMjIyMjIyMjIyMjIyMjIyMjIyMjIyMjIyMjIyMjIyMjIyMjIyMjL/wAARCAIAAgADASIAAhEBAxEB/8QAHwAAAQUBAQEBAQEAAAAAAAAAAAECAwQFBgcICQoL/8QAtRAAAgEDAwIEAwUFBAQAAAF9AQIDAAQRBRIhMUEGE1FhByJxFDKBkaEII0KxwRVS0fAkM2JyggkKFhcYGRolJicoKSo0NTY3ODk6Q0RFRkdISUpTVFVWV1hZWmNkZWZnaGlqc3R1dnd4eXqDhIWGh4iJipKTlJWWl5iZmqKjpKWmp6ipqrKztLW2t7i5usLDxMXGx8jJytLT1NXW19jZ2uHi4+Tl5ufo6erx8vP09fb3+Pn6/8QAHwEAAwEBAQEBAQEBAQAAAAAAAAECAwQFBgcICQoL/8QAtREAAgECBAQDBAcFBAQAAQJ3AAECAxEEBSExBhJBUQdhcRMiMoEIFEKRobHBCSMzUvAVYnLRChYkNOEl8RcYGRomJygpKjU2Nzg5OkNERUZHSElKU1RVVldYWVpjZGVmZ2hpanN0dXZ3eHl6goOEhYaHiImKkpOUlZaXmJmaoqOkpaanqKmqsrO0tba3uLm6wsPExcbHyMnK0tPU1dbX2Nna4uPk5ebn6Onq8vP09fb3+Pn6/9oADAMBAAIRAxEAPwD3+iiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKaZY16uo+ppv2iEdZo/++hS5l3FdElFR/aIT/wAto/8AvoUoljPSRT9DRzLuF0Poo60UxhRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRTJJo4V3SOqj3NJtLVhew+isybWY14hQv7ngVnzaldTceZsHonFc08XTjtqYyrwXmdBJNHEMySKv1NU5NXtU+6Wc+w/xrAJJOScmiuWWOm/hVjCWJk9kasmtuf9XCo/3jmq76rdv0cL/urVKisJYirLeRm6s31Jmu7h/vTyH/AIEaiLM3Uk/U0lFZOTe7M229wooopAFFFFACgkdCR9KlW6uE+7NIP+BGoaKak1sCbWxcTVLtP+Wm4f7QFWE1uQf6yJW/3TisuitY4irHaRaqzXU3o9Ytn+/vQ+4yP0q5HcQzf6uRW9gea5Wjp0reOOmviVzWOJktzrqK5uHULmH7spI9G5q/DrSniaMr7ryK6oYynLfQ2jiIPfQ1aKjiuIpxmKRW+nWpK6U01dGyd9gooopjCiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKjmnit03SuFH6mk2krsG7bklQXF3DbD944z/dHJNZV1q8kmVgBjX17n/Cs4ksSSSSe5riq41LSGpzTxCWkTRuNYlkyIVEa+vU1nM7OxZ2LE9yc0lFcE6s5v3mcspyluwooorMkKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAVWKkFSQR0Iq/b6vPFgSYkX34P51n0VcKkoO8WVGco7M6W3voLnhHw391uDVmuR6VoWuqzQ4WX94nv1Fd9LGp6TOmGIW0jeoqGC5iuV3RPn1HcVNXcmmro6U09UFFFFMYUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRTJZUhjLyMFUVhXmpSXJKJlIvTufrWNavGktdzOpVUNy9easkWUgw7/wB7sP8AGsaWV5nLyMWY9zTKK8qrWnUepwzqSnuFFFFYkBRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQA5HaNwyMVYdCK17TVw2EuMKf746fjWNRWtKtOm7xLhUlB6HXAggEHIPeiucs9QltSF+/H3U9vpW9BcR3Ee+NsjuO4r1aOIjVWm5206qn6ktFFFbmoUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAVBdXcdpHuc5Y/dUdTTL29S0j/AL0h+6tc9LK80hkkYljXJiMSqfux3MKtbk0W4+5upLqTdIeOyjoKhoorym3J3Zwttu7CiiikAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAVLBPJbyB42we/oaiopptO6BO2qOks72O7Tj5ZB1WrVcmjtG4dGKsOhFb9jfrdLtbCyjqPX3Feph8Tz+7Lc7aVbm0e5dooorsOgKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACqt7epaR9jIfur/Wn3d0lpCXbljwq+prm5ZXnlaSQ5Y1yYnEezXLHcwrVeTRbiSSPLIXdiWPU02iivKbucIUUUUgCiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKVWZGDKSGHIIpKKAOhsL5bpNrYEoHI9fertcmjtG4dCQwOQRXRWV4t3FngOPvLXq4bEc65ZbnbRq83uvctUUUV2HQFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUyWVIYmkc4VRT65/Ur37TLsQ/ukPHufWsa9ZUo36mdSooK5Xurl7qYyN06AegqGiivFbcndnnNtu7CiiikAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFSQTvbzLIh5Hb1FR0U02ndAnbVHUwTpcQrIh4Pb0NS1zmn3htZ/mP7tuGHp710YIIBByDXs4esqsb9T0KVTnXmFFFFbmoUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUVHPMsELSv0UfnSbSV2DdtSjqt55UfkIfncc+wrDp8srTStI5yzHNMrxa9V1J3PNqT55XCiiisSAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKy9c1y20SzM0x3StxHEDy5/wAPejXNcttEszNMd0rcRxA8uf8AD3ryjUdRudUvHurp90jdB2Ueg9q3pUufV7HHisUqS5Y7noPhnxcuqubS92R3RJKEcK49Pr/OuqrwtWKsGUkMDkEdRXo/hTxWNQVbG+cC7AwjnpL/APZfzqq1G3vRMsLi+b3J7nW0UUVzHohRRRQAUUUUAFbOkXe5fs7nkcp9PSsanI7RurocMpyDWtGq6c+ZF05uErnWUVDbTrc26yr36j0NTV7aaauj0U7q6CiiimMKKKKACiiigAooooAKKKKACiiigArE1e68yUQKflTlvc1q3c4trZ5D1HAHqa5gksxYnJJyTXDjatlyLqc2InZcqEooorzDjCiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigArL1zXLbRLMzTHdK3EcQPLn/D3o1zXLbRLMzTHdK3EcQPLn/D3ryjUdRudUvHurp90jdB2Ueg9q3pUufV7HHisUqS5Y7hqOo3OqXj3V0+6Rug7KPQe1VaKK7kraI8Ztt3YUqsVYMpIYHII6ikooEekeFPFY1BVsb5wLsDCOekv/wBl/OutrwtWKsGUkMDkEdRXo/hTxWNQVbG+cC7AwjnpL/8AZfzrjrUbe9E9XCYvm9ye51tFFFcx6IUUUUAFFFFAGhpV15Nx5TH5JOPoa3q5EHByK6ayuPtNqr/xDhvrXpYKrdcjOvDz05WWKKKK7zqCiiigAooooAKKKKACiiigAoopksgiieRuijNJu2rAx9YuN8ywg8JyfrWZTndpJGdjlmOTTa8OrPnm5HmTlzSbCiiisyQooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigArL1zXLbRLMzTHdK3EcQPLn/D3o1zXLbRLMzTHdK3EcQPLn/D3ryjUdRudUvHurp90jdB2Ueg9q3pUufV7HHisUqS5Y7hqOo3OqXj3V0+6Rug7KPQe1VaKK7kraI8Ztt3YUUUUCCiiigApVYqwZSQwOQR1FJRQB6R4U8VjUFWxvnAuwMI56S//AGX8662vC1YqwZSQwOQR1Fej+FPFY1BVsb5wLsDCOekv/wBl/OuOtRt70T1cJi+b3J7nW0UUVzHohRRRQAVoaRceVcmMn5ZOPxrPpVYqwYHBByDV05uElJFQlyyTOtoqO3lE8CSj+IZqSvdTTV0eknfUKKKKYwooooAKKKKACiiigArN1mbZbrEDy5yfoK0q53U5vNvn54T5R/n61zYufLTt3Ma8rQ9SnRRRXjnAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFZeua5baJZmaY7pW4jiB5c/4e9Gua5baJZmaY7pW4jiB5c/4e9eUajqNzql491dPukboOyj0HtW9Klz6vY48VilSXLHcNR1G51S8e6un3SN0HZR6D2qrRRXclbRHjNtu7CiiigQUUUUAFFFFABRRRQAV1vhPws9/ImoXgZLVTujXoZCO/wBKTwp4UOost9fIRaA5RD1lP+H869IVQihVACgYAA4ArmrVre7E9HCYXm9+ewtFFFcZ6oUUUUAFFFFAGzos2Y3hJ+6dw+latc3p83k3sZ7Mdp/Gukr18HPmp27Hdh5XhbsFFFFdRuFFFFABRRRQAUUUUAMlcRRPIeigmuVYlmLHqTk1v6rJ5diw7uQv+fyrn68zHSvJR7HHiZe8kFFFFcJzBRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFZeua5baJZmaY7pW4jiB5c/4e9Gua5baJZmaY7pW4jiB5c/4e9eUajqNzql491dPukboOyj0HtW9Klz6vY48VilSXLHcNR1G51S8e6un3SN0HZR6D2qrRRXclbRHjNtu7CiiigQUUUUAFFFFABRRRQAV1nhTwodRZb6+Qi0ByiHrKf8P50eFPCh1Flvr5CLQHKIesp/w/nXpCqEUKoAUDAAHAFc1atb3Yno4TCc3vz2BVCKFUAKBgADgCloorjPVCiiigAooooAKKKKADoc11UEnnW8cn95Qa5Wt7R5N9nt7oxH9a7cDK03HudGGlaVjQooor1DtCiiigAooooAKKKKAMfW5OYo/qxrJq9qz7r9h/dUD+v9ao14uIlzVWedVd5sKKKKwMwooooAKKKKACiiigAooooAKKKx9d8RWuhRJ5oMszn5YlPOO5PoKaTbsiZSUFzS2Niiq9jfW+o2iXVrIHicde4PofQ1YpNWGmmroKKKKBhRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABWXrmuW2iWZmmO6VuI4geXP+HvRrmuW2iWZmmO6VuI4geXP+HvXlGo6jc6pePdXT7pG6Dso9B7VvSpc+r2OPFYpUlyx3DUdRudUvHurp90jdB2Ueg9qq0UV3JW0R4zbbuwooooEFFFFABRRRQAUUUUAFdZ4U8KHUWW+vkItAcoh6yn/D+dHhTwodRZb6+Qi0ByiHrKf/AIn+dekKoRQqgBQMAAcAVzVq1vdiejhMJze/PYFUIoVQAoGAAOAKWiiuM9UKKKKACiiigAooooAKKKKACtTRHxNLH6qD+X/66y6uaW+y/j9GyP0rbDy5asWXSdpo6KiiivbPSCiiigAooooAKKKKAOYvW33sx/2yPy4qCnStuldvViabXgSd5Nnlyd22FFFFSIKKKKACiiigAooooAKKKxfEPiGDQ7XtJdOP3cWf1Pt/OnGLk7Imc1Bc0tg8Q+IYNDte0l04/dxZ/U+3868qu7ue+upLm5kMkrnLMaLu7nvrqS5uZDJK5yzGoa9ClSUF5niYjEOs/I1tB1640O73pl4HP72LPDD1Hoa9Xsb631G0S6tZA8Tjr3B9D6GvEq1tB1640O73pl4HP72LPDD1HoaitR5tVuaYXFOm+WW35Hr9FV7G+t9RtEurWQPE469wfQ+hqxXC1Y9hNNXQUUUUDCiiigAooooAKKKKACiiigArL1zXLbRLMzTHdK3EcQPLn/D3o1zXLbRLMzTHdK3EcQPLn/D3ryjUdRudUvHurp90jdB2Ueg9q3pUufV7HHisUqS5Y7hqOo3OqXj3V0+6Rug7KPQe1VaKK7kraI8Ztt3YUUUUCCiiigAooooAKKKKACus8KeFDqLLfXyEWgOUQ9ZT/h/Ojwp4UOost9fIRaA5RD1lP+H869IVQihVACgYAA4ArmrVre7E9HCYTm9+ewKoRQqgBQMAAcAUtFFcZ6oUUUUAFFFFABRRRQAUUUUAFFFFABU1q2y7hb0cfzqGlBwwPoacXZpgnZ3Otooor6A9UKKKKACiiigApGOFJ9BS02XiJ/8AdNJ7Azk6KKK+fPKCiiigAooooAKKKKACiisXxD4hg0O17SXTj93Fn9T7fzpxi5OyJnNQXNLYPEPiGDQ7XtJdOP3cWf1Pt/OvKru7nvrqS5uZDJK5yzGi7u5766kubmQySucsxqGvQpUlBeZ4mIxDrPyCiiitDmCiiigDW0HXrjQ7vemXgc/vYs8MPUehr1exvrfUbRLq1kDxOOvcH0Poa8SrW0HXrjQ7vemXgc/vYs8MPUehrCtR5tVuduFxTpvllt+R6/RVexvrfUbRLq1kDxOOvcH0PoasVwtWPYTTV0FFFFAwooooAKKKKACsvXNcttEszNMd0rcRxA8uf8PejXNcttEszNMd0rcRxA8uf8PevKNR1G51S8e6un3SN0HZR6D2relS59XsceKxSpLljuGo6jc6pePdXT7pG6Dso9B7VVooruStojxm23dhRRRQIKKKKACiiigAooooAK6zwp4UOost9fIRaA5RD1lP+H86PCnhQ6iy318hFoDlEPWU/wCH869IVQihVACgYAA4ArmrVre7E9HCYTm9+ewKoRQqgBQMAAcAUtFFcZ6oUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAdXEcxIfVRT6jt+baI/7A/lUlfQR2R6i2CiiimMKKKKACmS/6p/900+kYZUj1FJ7AclRRRXz55QUUUUAFFFFABRRRQBi+IfEMGh2vaS6cfu4s/qfb+deVXd3PfXUlzcyGSVzlmNbfi3SL6x1N7m4ke4inbKTH/0E+hFc9XfRhGMbo8TF1Zznyy0S6BRRRWxyBRRRQAUUUUAFFFFAGtoOvXGh3e9MvA5/exZ4Yeo9DXq9jfW+o2iXVrIHicde4PofQ14lWtoOvXGh3e9MvA5/exZ4Yeo9DWFajzarc7cLinTfLLb8j1+iq9jfW+o2iXVrIHicde4PofQ1YrhasewmmroKKKKBhWXrmuW2iWZmmO6VuI4geXP+HvRrmuW2iWZmmO6VuI4geXP+HvXlGo6jc6pePdXT7pG6Dso9B7VvSpc+r2OPFYpUlyx3DUdRudUvHurp90jdB2Ueg9qq0UV3JW0R4zbbuwooooEFFFFABRRRQAUUUUAFdZ4U8KHUWW+vkItAcoh6yn/D+dHhTwodRZb6+Qi0ByiHrKf8P516QqhFCqAFAwABwBXNWrW92J6OEwnN789gVQihVACgYAA4ApaKK4z1QooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKAOqg4t4h/sD+VSU2IYiQeiinV9BHZHqLYKKKKYwooooAKKKKAOTlXbK6+jEU2p71dl7MP9sn86grwJK0mjy5KzaCiiipEFFFFABRRRQBDd2kF9ayW1zGJInGGU15X4i8Oz6HdZGZLRz+7l/off+detVDd2kF9ayW1zGJInGGU1rSquD8jmxGHVZeZ4hRW34i8Oz6HdZGZLRz+7l/off+dYld8ZKSujxJwcHyy3CiiimSFFFFABRRRQAUUUUAa2g69caHd70y8Dn97Fnhh6j0Ner2N9b6jaJdWsgeJx17g+h9DXiVa2g69caHd70y8Dn97Fnhh6j0NYVqPNqtztwuKdN8stvyPX6y9c1y20SzM0x3StxHEDy5/w96r3virTrXR0v45BL5o/dRg/Mzeh9Md68w1HUbnVLx7q6fdI3QdlHoPasKVFyd3sdmJxSpq0NWw1HUbnVLx7q6fdI3QdlHoPaqtFFdyVtEeO227sKKKKBBRRRQAUUUUAFFFFABXWeFPCh1Flvr5CLQHKIesp/wAP50eFPCh1Flvr5CLQHKIesp/w/nXpCqEUKoAUDAAHAFc1atb3Yno4TCc3vz2BVCKFUAKBgADgCloorjPVCiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKVRuYD1OKSprRd95Cv+2P504q7SBK7sdRRRRX0B6oUUUUAFFFFABRRRQBz+rJtv2P95Qf6f0qjWtracxSfVTWTXi4iPLVkjzqqtNhRRRWBmFFFFABRRRQAUUUUAQ3dpBfWr21zGJInGGU15X4i8Oz6HdZGZLRz+7l/off+detVDd2kF9ayW1zGJInGGU1rSquD8jmxGHVZeZ4hRW34i8Oz6HdZGZLRz+7l/off+dYld8ZKSujxJwcHyy3CiiimSFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAV1nhTwodRZb6+Qi0ByiHrKf8P50eFPCh1Flvr5CLQHKIesp/wAP516QqhFCqAFAwABwBXNWrW92J6OEwnN789gVQqhVACgYAHQUtFFcZ6oUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAVd0pN9+h/ugmqVauiR5klk9AF/wA/lW2HjzVYo0pK80bNFFFe2eiFFFFABRRRQAUUUUAUdVj32LHuhDf5/Oufrq5UEsToejAiuVYFWKngg4NeZjo2kpdzjxMfeTEooorhOYKKKKACiiigAooooAKKKKAIbu0gvrWS2uYxJE4wymvK/EXh2fQ7rIzJaOf3cv8AQ+/869aqG7tIL61ktrmMSROMMprWlVcH5HNiMOqy8zxCitvxF4dn0O6yMyWjn93L/Q+/86xK74yUldHiTg4PlluFFFFMkKKKKACiiigAooooAKKKKACiiigAooooAK6zwp4UOost9fIRaA5RD1lP+H86PCnhQ6iy318hFoDlEPWU/wCH869IVQihVACgYAA4ArmrVre7E9HCYTm9+ewKoRQqgBQMAAcAUtFFcZ6oUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFb+kR7LIN3dif6VggEkAdTXVQxiKFIx/CoFduBjebl2OjDRvJsfRRRXqHaFFFFABRRRQAUUUUAFc7qcPlXz4HD/ADCuirN1mHfbrKByhwfoa5sXDmp37GNeN4ehh0UUV45wBRRRQAUUUUAFFFFABRRRQAUUUUAQ3dpBfWsltcxiSJxhlNeV+IvDs+h3WRmS0c/u5f6H3/nXrVQ3dpBfWsltcxiSJxhlNa0qrg/I5sRh1WXmeIUVt+IvDs+h3WRmS0c/u5f6H3/nWJXfGSkro8ScHB8stwooopkhRRRQAUUUUAFFFFABRRRQAV1nhTwodRZb6+Qi0ByiHrKf8P50eFPCh1Flvr5CLQHKIesp/wAP516QqhFCqAFAwABwBXNWrW92J6OEwnN789gVQihVACgYAA4ApaKK4z1QooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKALemw+depkcL8x/CujrM0aHbC8xHLnA+grTr18JDlp37nfQjaHqFFFFdRsFFFFABRRRQAUUUUAFMljEsTxt0YYp9FDV9GByciNHIyMMMpwabWnrFvsmWYDh+D9azK8KrDkm4nmTjyyaCiiisyQooooAKKKKACiiigAooooAKKKKAIbu0gvrWS2uYxJE4wymvK/EXh2fQ7rIzJaOf3cv9D7/AM69aqG7tIL61ktrmMSROMMprWlVcH5HNiMOqy8zxCitvxF4dn0O6yMyWjn93L/Q+/8AOsSu+MlJXR4k4OD5ZbhRRRTJCiiigAooooAK6zwp4UOost9fIRaA5RD1lP8Ah/Ojwp4UOost9fIRaA5RD1lP+H869IVQihVACgYAA4ArmrVre7E9HCYTm9+ewKoRQqgBQMAAcAUtFFcZ6oUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABSopd1RRlmOBSVpaPb75zMR8qdPrWlKDnNRRUI80kjZhjEMKRr0UYp9FFe4lZWR6aVgooopgFFFFABRRRQAUUUUAFFFFAEN3ALm2eM9SOD6GuYYFWKkYIOCK62sTV7Xy5ROo+V+G9jXDjaV1zroc2IhdcyMyiiivMOMKKKKACiiigAooooAKKKKACiiigAooooAhu7SC+tZLa5jEkTjDKa8r8ReHZ9DusjMlo5/dy/0Pv/OvWqhu7SC+tZLa5jEkTjDKa1pVXB+RzYjDqsvM8Qorb8ReHZ9DusjMlo5/dy4/Q+/86xK74yUldHiTg4PlluFFFFMkK6zwp4UOost9fIRaA5RD1lP+H86PCnhQ6iy318hFoDlEPWU/4fzr0hVCKFUAKBgADgCuatWt7sT0cJhOb357AqhFCqAFAwABwBS0UVxnqhRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFACgFiABkngCumtLcW1skffqx9TWVpFr5kxnYfKnT3NblengqVlzvqdmHhZczCiiiu46QooooAKKKKACiiigAooooAKKKKACo54VnhaJujD8qkopNJqzBq+hyksTQytG4wynFMrc1Wz82Pz0HzoOR6isOvFr0nTnY82pDklYKKKKxICiiigAooooAKKKKACiiigAooooAKKKKAIbu0gvraS2uYxJE4wymvK/EXh2fQ7nIzJaOf3cv9D7/AM69aqG7tIL62ktrmMSROMMprWlVcH5HNiMOqy8zxCus8KeFDqLLfXyEWgOUQ9ZT/h/OtKy8BLFrDvcyiWxQ7o1/if2b6frXbKoRQqgBQMAAcAVtVrq1onJhsG781RfIFUIoVQAoGAAOAKWiiuQ9QKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKfFE00qxoMsxwKZW5pNn5UfnuPncfKPQVtRpOpOxdOHPKxeghW3gWJeijr61JRRXtJJKyPRStogooopjCiiigAooooAKKKKACiiigAooooAKKKKACuf1Ky+zS70H7pzx7H0roKZLEk0TRuMqaxr0VVjbqZ1afOrHKUVNdWz2sxjbp1B9RUNeLJOLszzmmnZhRRRSAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiprW2e6mEa9O59BTScnZAk27IsabZ/aZt7j90h59z6V0FMiiSGJY0GFWn17VCiqUbdT0aVNQVgooorY0CiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAgu7VLuEo3DDlW9DXNyxPBIY5BhhXV1VvbJbuPsJB91v6VyYnD+0XNHcwrUudXW5zdFOkjeKQo6kMOopteU1Y4QooopAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUU6ON5ZAiKWY9BTSuAsUTzyrHGMsa6S0tUtIQi8seWb1NMsrJLSP1kP3m/pVqvVw2H9muaW53UaXJq9wooorrNwooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAq3tkl2n92Qfdb/GuelieCQxyLhhXV1BdWkd3HtcYYfdYdRXJiMMqnvR3MKtHn1W5zFFTXNrLaybZBx2YdDUNeVKLi7M4WmnZhRRRSAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKmtrWW6k2xj6segppOTsgSbdkMiieaQRxrljXQ2VklpH/AHpD95v8Kfa2kdpHtQZY/eY9TU9erh8MqfvS3O6lR5NXuFFFFdZuFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAMliSaMpIoZTWFe6bJbZePLxevcfWugorGtQjVWu5nUpxmtTkaK3LzSkly8OEf07H/CsaWKSFykilWHrXlVaE6b1OGdOUNxlFFFYkBRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUU+KJ5nCRqWY9hWzZ6SkWHnw7/AN3sP8a2pUZ1HoXCnKexRs9NkucO+Ui9e5+lbsUSQxhI1CqKfRXq0aEaS03O6nSUNgooorY0CiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKjmgjnTZKgYfyqSik0mrMGr7mJdaRJHloDvX+6eo/xrNIKkhgQR1BrrahntYbkYkQE9iOoriq4JPWGhzTw6esTl6K07jR5Ey0Lbx6Hg1nPG8bbXUqfQjFcE6U4fEjllCUd0NooorMkKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKciNIwVFLMewGa0LfR5XwZmEa+g5NaQpTm/dRUYSlsjOALEAAknsK0bXSJJMNOfLX07n/CtW3tIbYfu0Gf7x5NT130sElrPU6oYdLWRHDBFbptiQKO/qakoortSSVkdCVtgooopjCiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKKKKACiiigAooooAKZJFHKu2RFYehFPooavowM2bRon5iYxn0PIrPm0y6i5Cbx6pz+ldFRXNPCU5baGMqEH5HJMpU4YEH0IpK6t4o5RiRFYe4zVWTSrWTorIf8AZNcssDJfC7mMsNLoznqK1pNEP/LOb8GFV30m6XoFf/db/GsJYarHoZOjNdCjRVhrK6TrA/4DNRNFIv3kYfUVk4yW6IcWt0MoooqRBRRRQAUU4RyN91GP0FSrZXL9IH/EYqlGT2Q1FvYgoq8mk3bdVVf95v8ACrCaI3/LSYD2UVpHD1ZbRLVKb6GTSgFjgAk+grfj0m1TqrOf9o/4VbjijiGI0VR7DFdEcDN/E7GkcNLqzn4dNupcHy9g9X4rQh0aJcGZy59BwK06K6YYSnHfU3jQgvMZHDHCu2NFUewp9FFdKSWiNrWCiiimAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAhAPUA0nlp/cX8qdRSsgG+Wg/gX8qUKB0AFLRRZBYKKKKYBRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQAUUUUAFFFFABRRRQB/9k=;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="75" vertex="1">
          <mxGeometry x="154" y="25" width="20" height="17" as="geometry" />
        </mxCell>
        <mxCell id="28" style="vsdxID=194;fillColor=none;gradientColor=none;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="551" y="418" width="133" height="89" as="geometry" />
        </mxCell>
        <mxCell id="29" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;&amp;lt;mask&amp;gt;&lt;/b&gt;&lt;/font&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;&#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=195;fillColor=#dae2f3;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="28" vertex="1">
          <mxGeometry width="80" height="22" as="geometry" />
        </mxCell>
        <mxCell id="30" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;R (S)&lt;/b&gt;&lt;/font&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;&#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=196;fillColor=#dae2f3;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="28" vertex="1">
          <mxGeometry x="80" width="52" height="22" as="geometry" />
        </mxCell>
        <mxCell id="31" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;mathematic&lt;/font&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=197;fillColor=#dae2f3;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="28" vertex="1">
          <mxGeometry y="22" width="80" height="22" as="geometry" />
        </mxCell>
        <mxCell id="32" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;1 (1/1)&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=198;fillColor=#dae2f3;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="28" vertex="1">
          <mxGeometry x="80" y="22" width="52" height="22" as="geometry" />
        </mxCell>
        <mxCell id="33" style="vsdxID=199;fillColor=#dae2f3;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="28" vertex="1">
          <mxGeometry y="44" width="80" height="22" as="geometry" />
        </mxCell>
        <mxCell id="34" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;...&#xa;&lt;/font&gt;&lt;/p&gt;" style="text;vsdxID=199;fillColor=none;gradientColor=none;rotation=270.05;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;verticalAlign=middle;align=center;;html=1;" parent="33" vertex="1">
          <mxGeometry y="-0.21" width="80.79" height="22.21" as="geometry" />
        </mxCell>
        <mxCell id="35" style="vsdxID=200;fillColor=#dae2f3;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="28" vertex="1">
          <mxGeometry x="80" y="44" width="52" height="22" as="geometry" />
        </mxCell>
        <mxCell id="36" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;...&#xa;&lt;/font&gt;&lt;/p&gt;" style="text;vsdxID=200;fillColor=none;gradientColor=none;rotation=270.05;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;verticalAlign=middle;align=center;;html=1;" parent="35" vertex="1">
          <mxGeometry y="-0.21" width="52.44" height="22.21" as="geometry" />
        </mxCell>
        <mxCell id="37" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;physics&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=201;fillColor=#dae2f3;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="28" vertex="1">
          <mxGeometry y="66" width="80" height="22" as="geometry" />
        </mxCell>
        <mxCell id="38" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;7 (1/7)&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=202;fillColor=#dae2f3;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="28" vertex="1">
          <mxGeometry x="80" y="66" width="52" height="22" as="geometry" />
        </mxCell>
        <mxCell id="106" value="" style="verticalAlign=middle;align=center;vsdxID=416;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLbjsIgFPwVct6hF60rCeVfiKUtWbY0p6j1761gFX3ZTdwnwgyZGc4ZMfVq1GTy6L712TS+r8EMvUbjQYrWoe7QHYdGilH5Xoofd9JkrqHIgVxuRw6ZFNYMAeV/QBUeCAYFVmyAYGDYDqJqfLrnrFq4marZTBSdV964oYaFtQo7TRcR2lrVBWg6az0+ronxKrfob79Sb87KMlpztqsgCUnzz22fUi9ZfgOf4ao1G4/Z0l98nC6d8Os69veZFAXblPC25X9YRtqCLNapNdbG7t2wtG5ZKKa8Ag==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="390" y="144" width="106" height="101" as="geometry" />
        </mxCell>
        <mxCell id="107" style="vsdxID=417;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="440" y="171" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="108" style="vsdxID=418;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="418" y="200" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="109" style="vsdxID=419;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="462" y="200" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="110" style="vsdxID=422;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="405" y="227" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="111" style="vsdxID=423;fillColor=#f7cbac;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="431" y="227" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="112" style="vsdxID=424;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="462" y="227" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="114" value="" style="verticalAlign=middle;align=center;vsdxID=441;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLbjsIgFPwVct6hF60rCeVfiKUtWbY0p6j1761gFX3ZTdwnwgyZGc4ZMfVq1GTy6L712TS+r8EMvUbjQYrWoe7QHYdGilH5Xoofd9JkrqHIgVxuRw6ZFNYMAeV/QBUeCAYFVmyAYGDYDqJqfLrnrFq4marZTBSdV964oYaFtQo7TRcR2lrVBWg6az0+ronxKrfob79Sb87KMlpztqsgCUnzz22fUi9ZfgOf4ao1G4/Z0l98nC6d8Os69veZFAXblPC25X9YRtqCLNapNdbG7t2wtG5ZKKa8Ag==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="664" y="144" width="106" height="101" as="geometry" />
        </mxCell>
        <mxCell id="115" style="vsdxID=442;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="714" y="171" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="116" style="vsdxID=443;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="692" y="200" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="39" style="vsdxID=203;fillColor=none;gradientColor=none;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="742" y="418" width="133" height="89" as="geometry" />
        </mxCell>
        <mxCell id="40" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;&amp;lt;mask&amp;gt;&lt;/b&gt;&lt;/font&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;&#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=204;fillColor=#e2efd9;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="39" vertex="1">
          <mxGeometry width="81" height="22" as="geometry" />
        </mxCell>
        <mxCell id="41" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;R (S)&lt;/b&gt;&lt;/font&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;&#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=205;fillColor=#e2efd9;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="39" vertex="1">
          <mxGeometry x="81" width="51" height="22" as="geometry" />
        </mxCell>
        <mxCell id="42" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;mathematic&lt;/font&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=206;fillColor=#e2efd9;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="39" vertex="1">
          <mxGeometry y="22" width="81" height="22" as="geometry" />
        </mxCell>
        <mxCell id="43" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;2 (1/2)&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=207;fillColor=#e2efd9;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="39" vertex="1">
          <mxGeometry x="81" y="22" width="51" height="22" as="geometry" />
        </mxCell>
        <mxCell id="44" style="vsdxID=208;fillColor=#e2efd9;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="39" vertex="1">
          <mxGeometry y="44" width="81" height="22" as="geometry" />
        </mxCell>
        <mxCell id="45" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;...&#xa;&lt;/font&gt;&lt;/p&gt;" style="text;vsdxID=208;fillColor=none;gradientColor=none;rotation=270.05;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;verticalAlign=middle;align=center;;html=1;" parent="44" vertex="1">
          <mxGeometry y="-0.21" width="81.74" height="22.21" as="geometry" />
        </mxCell>
        <mxCell id="46" style="vsdxID=209;fillColor=#e2efd9;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="39" vertex="1">
          <mxGeometry x="81" y="44" width="51" height="22" as="geometry" />
        </mxCell>
        <mxCell id="47" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;...&#xa;&lt;/font&gt;&lt;/p&gt;" style="text;vsdxID=209;fillColor=none;gradientColor=none;rotation=270.05;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;verticalAlign=middle;align=center;;html=1;" parent="46" vertex="1">
          <mxGeometry y="-0.21" width="51.48" height="22.21" as="geometry" />
        </mxCell>
        <mxCell id="48" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;physics&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=210;fillColor=#e2efd9;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="39" vertex="1">
          <mxGeometry y="66" width="81" height="22" as="geometry" />
        </mxCell>
        <mxCell id="49" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:14px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;9 (1/9)&#xa;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=211;fillColor=#e2efd9;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="39" vertex="1">
          <mxGeometry x="81" y="66" width="51" height="22" as="geometry" />
        </mxCell>
        <mxCell id="117" style="vsdxID=444;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="736" y="200" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="118" style="vsdxID=447;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="692" y="227" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="119" style="vsdxID=449;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="736" y="227" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="120" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:top;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;Remaining &#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:top;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;Entity List&#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=top;align=center;vsdxID=455;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLbjsIgFPwVct6hF22VhPIvRGlLZEtzym71763gBX0wJu4TYQ6ZmcOMmHo1ajJ5dAc9m73vGzBDr9F4kKJ1qDt0v8NeilH5Xoof96fJsYEiB3K6HDlkUlgzBJR/gCrcEQwMrKiBYJiweg2RNr7dclatFoSqo5koOq+8cUMDy9Qq7DRdWGhrVRegadZ6vF8T5RvdIrDepOKclWXU5qyuIHFJ8+9lr1QvVt5jD2fVzRiPxtIVvraWfu9zGJvtNYyClRxeMv6HJNIOZLFMrbE2Nu+CpWXLQi3lGQ==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="779" y="144" width="106" height="101" as="geometry" />
        </mxCell>
        <mxCell id="121" style="vsdxID=456;fillColor=#bdd7ee;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="838" y="206" width="13" height="12" as="geometry" />
        </mxCell>
        <mxCell id="122" style="vsdxID=457;fillColor=#bdd7ee;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="813" y="225" width="13" height="12" as="geometry" />
        </mxCell>
        <mxCell id="123" style="vsdxID=458;fillColor=#bdd7ee;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="838" y="225" width="13" height="12" as="geometry" />
        </mxCell>
        <mxCell id="124" style="vsdxID=461;fillColor=#f7cbac;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="813" y="205" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="126" style="vsdxID=480;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);dashed=1;strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="656" y="137" width="238" height="117" as="geometry" />
        </mxCell>
        <mxCell id="190" style="vsdxID=784;rotation=60;fillColor=none;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#ff0000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="405" y="203" width="52" height="31" as="geometry" />
        </mxCell>
        <mxCell id="50" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;Ensemble&#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=212;fillColor=#bdd7ee;gradientColor=none;shape=stencil(rZLhjoMgEIRfhex/USNoTZB3IS0qKSdmpa19+6o0LWkvlybXX4RhM99mGDH1atRk8uiO+mIOvm/ADL1G40GK1qHu0J2GgxSj8r0UP+6sydxASXkF5NpAnmWQSmHNsOl1QVnx0YPCPcHgVALB5YHVtM5hHV5H1lG+HHOiZjMl6Lzyxg0NLJpV2OlkcUhaq7pNmi5aj49rBI68IiqndXWncsoC9bniF7CxWSQ/cvtDfSaT5/cdS8qqbcfv5fJbKhXNdoHIC7pj8PbT/6a+9iYNtWqNtaGDqxbXLt0KKm8=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="593" y="385" width="133" height="17" as="geometry" />
        </mxCell>
        <mxCell id="220" style="vsdxID=822;edgeStyle=none;startArrow=none;endArrow=none;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.48120300751879697;exitY=-0.011235955056179775;exitDx=0;exitDy=0;exitPerimeter=0" parent="1" source="39" target="219" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="806" y="417" as="sourcePoint" />
            <mxPoint x="660" y="410" as="targetPoint" />
            <Array capacity="4" as="points">
              <mxPoint x="806" y="410.25" />
            </Array>
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="222" style="vsdxID=821;edgeStyle=none;startArrow=none;endArrow=none;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.45112781954887216;exitY=-0.011235955056179775;exitDx=0;exitDy=0;exitPerimeter=0" parent="1" source="17" target="221" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="463" y="417" as="sourcePoint" />
            <mxPoint x="660" y="410" as="targetPoint" />
            <Array capacity="4" as="points">
              <mxPoint x="463" y="409.86" />
            </Array>
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="191" style="vsdxID=785;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="384" y="281" width="149" height="89" as="geometry" />
        </mxCell>
        <mxCell id="192" style="vsdxID=790;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="396" y="288" width="25" height="25" as="geometry" />
        </mxCell>
        <mxCell id="193" style="vsdxID=791;fillColor=#f7cbac;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="396" y="340" width="25" height="25" as="geometry" />
        </mxCell>
        <mxCell id="194" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;i&gt;&lt;b&gt;: &lt;/b&gt;&lt;/i&gt;&lt;/font&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;i&gt;&lt;b&gt;physics&lt;/b&gt;&lt;/i&gt;&lt;/font&gt;&lt;font style=&quot;font-size:14px;font-family:Themed;color:#4672c4;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;&#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=793;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="410" y="290" width="88" height="23" as="geometry" />
        </mxCell>
        <mxCell id="195" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;i&gt;&lt;b&gt;: geometry&lt;/b&gt;&lt;/i&gt;&lt;/font&gt;&lt;font style=&quot;font-size:14px;font-family:Themed;color:#4672c4;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;&#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=800;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="403" y="340" width="124" height="23" as="geometry" />
        </mxCell>
        <mxCell id="208" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:top;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:25px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;Ensemble-based Content Filter&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=top;align=center;vsdxID=846;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="340" y="99" width="551" height="36" as="geometry" />
        </mxCell>
        <mxCell id="224" style="vsdxID=820;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.5037593984962406;exitY=0;exitDx=0;exitDy=0;exitPerimeter=0" parent="1" source="50" target="223" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="660" y="385" as="sourcePoint" />
            <mxPoint x="660" y="369" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-13" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-305" value="" style="group" parent="1" connectable="0" vertex="1">
          <mxGeometry x="505" y="144" width="106" height="101" as="geometry" />
        </mxCell>
        <mxCell id="102" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:top;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;Remaining &#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:top;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;Entity List&#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=top;align=center;vsdxID=432;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLbjsIgFPwVct6hF22VhPIvRGlLZEtzym71763gBX0wJu4TYQ6ZmcOMmHo1ajJ5dAc9m73vGzBDr9F4kKJ1qDt0v8NeilH5Xoof96fJsYEiB3K6HDlkUlgzBJR/gCrcEQwMrKiBYJiweg2RNr7dclatFoSqo5koOq+8cUMDy9Qq7DRdWGhrVRegadZ6vF8T5RvdIrDepOKclWXU5qyuIHFJ8+9lr1QvVt5jD2fVzRiPxtIVvraWfu9zGJvtNYyClRxeMv6HJNIOZLFMrbE2Nu+CpWXLQi3lGQ==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-305" vertex="1">
          <mxGeometry width="106" height="101" as="geometry" />
        </mxCell>
        <mxCell id="103" style="vsdxID=433;fillColor=#bdd7ee;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-305" vertex="1">
          <mxGeometry x="34" y="62" width="13" height="12" as="geometry" />
        </mxCell>
        <mxCell id="104" style="vsdxID=434;fillColor=#bdd7ee;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-305" vertex="1">
          <mxGeometry x="34" y="81" width="13" height="12" as="geometry" />
        </mxCell>
        <mxCell id="105" style="vsdxID=436;fillColor=#bdd7ee;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-305" vertex="1">
          <mxGeometry x="59" y="81" width="13" height="12" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-313" style="vsdxID=480;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);dashed=1;strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="384" y="136" width="238" height="117" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-360" style="vsdxID=237;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="-1040" y="216.5" width="346" height="173.5" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-361" value="&lt;font style=&quot;font-family: Calibri; color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;b style=&quot;&quot;&gt;&lt;font style=&quot;font-size: 24px;&quot;&gt;Output&lt;/font&gt;&lt;br&gt;&lt;/b&gt;&lt;/font&gt;" style="verticalAlign=middle;align=center;vsdxID=247;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="-932" y="212" width="139" height="40" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-362" value="&lt;p style=&quot;align:left;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;i&gt;&lt;br&gt;&lt;/i&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=left;vsdxID=270;fillColor=#fff2cc;gradientColor=none;shape=stencil(rZJfD4IgFMW/irvvIOp0uiHfhRUqi8Rd6d+3z8CKeqmtnhg/2DkH7uHzICeVzA7tTp301g0t6HFQqB0I3llUPdrDuBV8km4QfG+PKjm3kDFILreFQSq40aOnzRdU4ibBVQE9plUNQTNcrBta5Ash8qxngtZJp+3YwnJqJPaKLBKkM7L3aD4pNT22ke1dLhhEzg1lWfBuaJVDFJGw322fUi9ZPsFnuLJ+fExe+HTxO37OF//xyzhoUa7GGWUlvE35D+OIW5CGOnXamNC9G4vrlvpiiis=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="-1013" y="251.5" width="136" height="128" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-402" style="vsdxID=257;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="-1881" y="216.5" width="238" height="173.5" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-416" value="&lt;font style=&quot;font-family: Calibri; color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;b style=&quot;&quot;&gt;&lt;font style=&quot;font-size: 24px;&quot;&gt;Chain-of-Layer Module&lt;/font&gt;&lt;br&gt;&lt;/b&gt;&lt;/font&gt;" style="verticalAlign=middle;align=center;vsdxID=721;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="-1455" y="224.5" width="264" height="19" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-436" style="vsdxID=740;fillColor=none;gradientColor=none;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="-1387" y="294.5" width="57" height="54" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-437" value="" style="verticalAlign=middle;align=center;vsdxID=741;fillColor=#fff2cc;gradientColor=none;shape=stencil(rZLRjoMgFER/hdx30ca6CwnyL2SLSkrFXNlt9+8r0LV0H5om9olwIDMDd8Q8qEmT2aM76rM5+KEFMw4ajQcpOoe6R/c9HqSYlB+kOLkfTS4t7Cogv2GpoJTCmjFS/gJV+EUwUMo+gGA8oHUNSTVdZZw2gRTqYuYCnVfeuLGF5dQq7HWxiBSdVX1E81nrad1mxn9yi8H+M/dmUT54M8qT9S1ktd11VXpI8pzdg3GWgnG6j7nyF2yOlv9u5rqoV/U6iwb+DfgNc8gLUKYmdcbaVLvA8qaVsZPyCg==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-436" vertex="1">
          <mxGeometry width="57" height="54" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-438" style="vsdxID=742;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZBLDsMgDESvgrxHSRbdAXexGvNRaYgMbcjtm0BVddVVl/M0HulZZY8riVw43WgLc/EawuKJQwGjbGJynB7LbNSKxRt1T08SVcMIYtdwGWEwCvkquLYkuNOzMo2fkqgSa8iSU8ES0qJBHjAiO5LHtbQRXdvMG9H6jtOP7T8sD13Ihhi7/cm+hYf2GvMC);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-436" vertex="1">
          <mxGeometry x="26" y="6" width="7" height="7" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-439" style="vsdxID=743;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZBLDsMgDESvgrxHSRbdAXexGvNRaYgMbcjtm0BVddVVl/M0HulZZY8riVw43WgLc/EawuKJQwGjbGJynB7LbNSKxRt1T08SVcMIYtdwGWEwCvkquLYkuNOzMo2fkqgSa8iSU8ES0qJBHjAiO5LHtbQRXdvMG9H6jtOP7T8sD13Ihhi7/cm+hYf2GvMC);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-436" vertex="1">
          <mxGeometry x="14" y="21" width="7" height="7" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-440" style="vsdxID=744;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZBLDsMgDESvgrxHSRbdAXexGvNRaYgMbcjtm0BVddVVl/M0HulZZY8riVw43WgLc/EawuKJQwGjbGJynB7LbNSKxRt1T08SVcMIYtdwGWEwCvkquLYkuNOzMo2fkqgSa8iSU8ES0qJBHjAiO5LHtbQRXdvMG9H6jtOP7T8sD13Ihhi7/cm+hYf2GvMC);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-436" vertex="1">
          <mxGeometry x="37" y="21" width="7" height="7" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-441" style="vsdxID=747;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZBLDsMgDESvgrxHSRbdAXexGvNRaYgMbcjtm0BVddVVl/M0HulZZY8riVw43WgLc/EawuKJQwGjbGJynB7LbNSKxRt1T08SVcMIYtdwGWEwCvkquLYkuNOzMo2fkqgSa8iSU8ES0qJBHjAiO5LHtbQRXdvMG9H6jtOP7T8sD13Ihhi7/cm+hYf2GvMC);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-436" vertex="1">
          <mxGeometry x="14" y="36" width="7" height="7" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-442" style="vsdxID=748;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZBLDsMgDESvgrxHSRbdAXexGvNRaYgMbcjtm0BVddVVl/M0HulZZY8riVw43WgLc/EawuKJQwGjbGJynB7LbNSKxRt1T08SVcMIYtdwGWEwCvkquLYkuNOzMo2fkqgSa8iSU8ES0qJBHjAiO5LHtbQRXdvMG9H6jtOP7T8sD13Ihhi7/cm+hYf2GvMC);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-436" vertex="1">
          <mxGeometry x="37" y="36" width="7" height="7" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-443" style="vsdxID=750;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.5714285714285714;exitY=1;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.5714285714285714;entryY=-0.14285714285714285;entryDx=0;entryDy=0;entryPerimeter=0" parent="ZVaZIW3ceO06EkHoMhZQ-436" source="ZVaZIW3ceO06EkHoMhZQ-440" target="ZVaZIW3ceO06EkHoMhZQ-442" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="41" y="28" as="sourcePoint" />
            <mxPoint x="41" y="35" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-13" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-444" value="" style="vsdxID=749;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;align=center;exitX=0.42857142857142855;exitY=1;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.42857142857142855;entryY=-0.14285714285714285;entryDx=0;entryDy=0;entryPerimeter=0" parent="ZVaZIW3ceO06EkHoMhZQ-436" source="ZVaZIW3ceO06EkHoMhZQ-439" target="ZVaZIW3ceO06EkHoMhZQ-441" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="17" y="28" as="sourcePoint" />
            <mxPoint x="17" y="35" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="12" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-445" style="vsdxID=746;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.8571428571428571;exitY=0.7142857142857143;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.5714285714285714;entryY=-0.14285714285714285;entryDx=0;entryDy=0;entryPerimeter=0" parent="ZVaZIW3ceO06EkHoMhZQ-436" source="ZVaZIW3ceO06EkHoMhZQ-438" target="ZVaZIW3ceO06EkHoMhZQ-440" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="32" y="11" as="sourcePoint" />
            <mxPoint x="41" y="20" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="8" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-446" style="vsdxID=745;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.14285714285714285;exitY=0.7142857142857143;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.42857142857142855;entryY=-0.14285714285714285;entryDx=0;entryDy=0;entryPerimeter=0" parent="ZVaZIW3ceO06EkHoMhZQ-436" source="ZVaZIW3ceO06EkHoMhZQ-438" target="ZVaZIW3ceO06EkHoMhZQ-439" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="27" y="11" as="sourcePoint" />
            <mxPoint x="17" y="20" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-8" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-447" style="vsdxID=755;fillColor=none;gradientColor=none;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="-1870" y="308.5" width="217" height="73" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-448" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;b&gt;&lt;font face=&quot;Calibri&quot; style=&quot;font-size: 18px;&quot;&gt;&lt;font style=&quot;color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;i style=&quot;&quot;&gt;Build a taxonomy whose root concept is \(v_0\)&lt;/i&gt;&lt;/font&gt;&lt;font style=&quot;color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;i&gt;&amp;nbsp;&lt;/i&gt;&lt;/font&gt;&lt;font style=&quot;color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;i&gt;with the given&lt;/i&gt;&lt;/font&gt;&lt;font style=&quot;color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;i&gt; &lt;/i&gt;&lt;/font&gt;&lt;font style=&quot;color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;i&gt;entity &lt;/i&gt;&lt;/font&gt;&lt;font style=&quot;color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;i&gt;list \(\mathcal{V}\)&lt;/i&gt;&lt;/font&gt;&lt;font style=&quot;color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;i&gt;&lt;/i&gt;&lt;/font&gt;&lt;/font&gt;&lt;/b&gt;&lt;font style=&quot;color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;i style=&quot;&quot;&gt;&lt;b style=&quot;&quot;&gt;&lt;font face=&quot;T2COjT3ncuN_wm8N9ywp&quot; size=&quot;3&quot; style=&quot;&quot;&gt;...&lt;/font&gt;&lt;/b&gt;&lt;br&gt;&lt;/i&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=259;fillColor=#bdd7ee;gradientColor=none;shape=stencil(rZJfD4IgFMW/CrvvImZqbsh3YYXKInFX+vftUyyjHlpbPTEO7Jwf3MOHVvaKDA7tXp31zrUV6K5VqB0IXltUDdpjtxO8l64V/GBPilwqSBiQ67QwiAU3uvNq+YUqcUtwUmlZAsHxYFXSdQqz63y1YDRbj0okL3qI0DrptO0qGE+NxEZFo0lUG9l4aTgr1S/bIPhhNwXkr9nZPbrwFE9I9nvq4vRC8ll7ghXJnWxDcw8WPuFntvB7g9iEUZYuw8hyeBvxHyYRViCeu1RrY+biTVrYtdi3UtwA);strokeColor=#002060;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-447" vertex="1">
          <mxGeometry width="217" height="73" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-449" style="vsdxID=471;fillColor=none;gradientColor=none;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="-1845" y="248.5" width="103" height="28" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-450" value="&lt;p style=&quot;align:left;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-family: Calibri; color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;b style=&quot;&quot;&gt;&lt;font style=&quot;font-size: 18px;&quot;&gt;Entity List \(\mathcal{V}\)&lt;/font&gt;&lt;/b&gt;&lt;br&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=left;vsdxID=258;fillColor=#fee599;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-449" vertex="1">
          <mxGeometry width="103.00000000000001" height="28" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-451" value="&lt;font style=&quot;font-family: Calibri; color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;b style=&quot;&quot;&gt;&lt;font style=&quot;font-size: 24px;&quot;&gt;Input&lt;/font&gt;&lt;br&gt;&lt;/b&gt;&lt;/font&gt;" style="verticalAlign=middle;align=center;vsdxID=757;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="-1851" y="222.5" width="179" height="19" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-477" style="vsdxID=828;fillColor=none;gradientColor=none;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="-1845" y="276.5" width="167" height="28" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-478" value="&lt;p style=&quot;align:left;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-family: Calibri; color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;b style=&quot;&quot;&gt;&lt;font style=&quot;font-size: 18px;&quot;&gt;     Demo. \(d_1, \cdots, d_n\)&lt;/font&gt;&lt;/b&gt;&lt;br&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=left;vsdxID=829;fillColor=#fee599;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-477" vertex="1">
          <mxGeometry width="166.99999999999997" height="28" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-486" style="vsdxID=751;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeWidth=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=1;exitY=0.5;exitDx=0;exitDy=0;entryX=0;entryY=0.5;entryDx=0;entryDy=0;entryPerimeter=0" parent="1" source="nIato8iqnGkG7OKb6TYW-350" target="ZVaZIW3ceO06EkHoMhZQ-437" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="-1491" y="321.5" as="sourcePoint" />
            <mxPoint x="-1423" y="319.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-488" value="" style="vsdxID=272;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;align=center;exitX=1.0073529411764706;exitY=0.5;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0;entryY=0.5;entryDx=0;entryDy=0;entryPerimeter=0" parent="1" source="ZVaZIW3ceO06EkHoMhZQ-362" target="ZVaZIW3ceO06EkHoMhZQ-453" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="-844" y="315.5" as="sourcePoint" />
            <mxPoint x="-812" y="315.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-2" y="-1" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-540" style="vsdxID=471;fillColor=none;gradientColor=none;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="-1742" y="248.5" width="64" height="28" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-541" value="&lt;p style=&quot;align:left;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-family: Calibri; color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;b style=&quot;&quot;&gt;&lt;font style=&quot;font-size: 18px;&quot;&gt;Root \(v_0\)&lt;/font&gt;&lt;/b&gt;&lt;br&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=left;vsdxID=258;fillColor=#fee599;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-540" vertex="1">
          <mxGeometry width="64" height="28" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-554" value="&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;No&#xa;&lt;/b&gt;&lt;/font&gt;" style="vsdxID=754;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeWidth=3;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;align=center;exitX=1;exitY=0.501;exitDx=0;exitDy=0;exitPerimeter=0;" parent="1" source="nIato8iqnGkG7OKb6TYW-298" edge="1">
          <mxGeometry x="-0.5576" relative="1" as="geometry">
            <mxPoint x="-1107" y="319.5" as="sourcePoint" />
            <mxPoint x="-1560" y="320" as="targetPoint" />
            <Array as="points">
              <mxPoint x="-1082.87" y="319.5" />
              <mxPoint x="-1082.87" y="255.27999999999997" />
              <mxPoint x="-1580" y="255" />
              <mxPoint x="-1580" y="320" />
              <mxPoint x="-1570" y="320" />
            </Array>
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-555" value="&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;Yes&#xa;&lt;/b&gt;&lt;/font&gt;" style="vsdxID=752;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeWidth=3;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;align=center;exitX=1.003;exitY=0.503;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.002;entryY=0.527;entryDx=0;entryDy=0;entryPerimeter=0;" parent="1" source="nIato8iqnGkG7OKb6TYW-298" target="ZVaZIW3ceO06EkHoMhZQ-362" edge="1">
          <mxGeometry x="-0.0214" y="1" relative="1" as="geometry">
            <mxPoint x="-1180" y="320" as="sourcePoint" />
            <mxPoint x="-980" y="316" as="targetPoint" />
            <Array as="points">
              <mxPoint x="-1029.21" y="319.5" />
            </Array>
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-556" style="vsdxID=724;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeWidth=3;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=1;exitY=0.5029585798816568;exitDx=0;exitDy=0;exitPerimeter=0;" parent="1" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="-1643" y="319.49999999999994" as="sourcePoint" />
            <mxPoint x="-1560" y="320" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-689" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\mathcal{T}^{k}$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" parent="1" vertex="1">
          <mxGeometry x="-969" y="480.5" width="180" height="40" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-772" value="" style="endArrow=none;dashed=1;html=1;rounded=0;entryX=0.006;entryY=0.998;entryDx=0;entryDy=0;entryPerimeter=0;exitX=0.004;exitY=-0.006;exitDx=0;exitDy=0;exitPerimeter=0;strokeWidth=2;" parent="1" source="ZVaZIW3ceO06EkHoMhZQ-678" target="ZVaZIW3ceO06EkHoMhZQ-414" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="-1593" y="421" as="sourcePoint" />
            <mxPoint x="-1543" y="371" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-773" value="" style="endArrow=none;dashed=1;html=1;rounded=0;entryX=0.999;entryY=0.999;entryDx=0;entryDy=0;entryPerimeter=0;exitX=1;exitY=0.001;exitDx=0;exitDy=0;exitPerimeter=0;strokeWidth=2;" parent="1" source="ZVaZIW3ceO06EkHoMhZQ-678" target="ZVaZIW3ceO06EkHoMhZQ-414" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="-1887" y="430" as="sourcePoint" />
            <mxPoint x="-1529" y="385" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-298" value="&lt;p style=&quot;align:left;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-family: Calibri; color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;i style=&quot;border-color: var(--border-color); letter-spacing: 0px; background-color: initial;&quot;&gt;&lt;b style=&quot;&quot;&gt;&lt;font style=&quot;font-size: 24px;&quot;&gt;Check&lt;/font&gt;&lt;span style=&quot;font-size: 18px;&quot;&gt;:&lt;/span&gt;&lt;/b&gt;&lt;span style=&quot;font-size: 18px;&quot;&gt;&amp;nbsp;&lt;/span&gt;&lt;/i&gt;&lt;/font&gt;&lt;/p&gt;&lt;p style=&quot;align:left;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-family: Calibri; color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1;&quot;&gt;&lt;i style=&quot;border-color: var(--border-color); letter-spacing: 0px; background-color: initial;&quot;&gt;&lt;font style=&quot;font-size: 18px;&quot;&gt;Is the remaining entity list empty?&lt;/font&gt;&lt;/i&gt;&lt;i style=&quot;font-size: 16px;&quot;&gt;&lt;br&gt;&lt;/i&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=left;vsdxID=270;fillColor=#BDD7EE;gradientColor=none;shape=stencil(rZJfD4IgFMW/irvvIOp0uiHfhRUqi8Rd6d+3z8CKeqmtnhg/2DkH7uHzICeVzA7tTp301g0t6HFQqB0I3llUPdrDuBV8km4QfG+PKjm3kDFILreFQSq40aOnzRdU4ibBVQE9plUNQTNcrBta5Ash8qxngtZJp+3YwnJqJPaKLBKkM7L3aD4pNT22ke1dLhhEzg1lWfBuaJVDFJGw322fUi9ZPsFnuLJ+fExe+HTxO37OF//xyzhoUa7GGWUlvE35D+OIW5CGOnXamNC9G4vrlvpiiis=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="-1310" y="273" width="126" height="94" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-405" style="vsdxID=351;fillColor=none;gradientColor=none;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="-1167" y="295.5" width="48" height="48" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-406" style="vsdxID=352;fillColor=#74aa9c;gradientColor=none;shape=stencil(dZFRDoMgEESvYjiAItSoCXIXU7GQWjWILd6+woqlTfq15E12djKwRbazSBajp7t4qc7IBqlRCq0M4qyftLjpaR07zubWSM4e01MktkEYJVuDyCXFOco4u67a8RyEfeQ4LQuUWHI+N+JFS2GN7IQ6sm8PavSmZZHWlTfG36ZVnZICjHEwxWAZDtHAaBQrGIMCM8Ihxyl8LobQ+bFsIb27eISxFAiF3HVs/NPOH5xBpb0aBujfsbjyzH8OfwM=);strokeColor=none;spacingTop=-3;spacingBottom=-3;spacingLeft=-3;spacingRight=-3;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-405" vertex="1">
          <mxGeometry width="48" height="48" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-407" style="vsdxID=353;fillColor=#FFFFFF;gradientColor=none;shape=stencil(fVTtboMwDHwVlAdwkzifEvAu1UoHWtdOlG7t28/BoYXS7Z/lA99dfEl5brdfTXEe+tNH89PthrYS3bFt+m4Qdbk/9c17f7ocd3X5tR3auvw8fTfFtRLWgtSiuFVCgrRiU5dvlz5BqhKoIEEqY8VVV0JRidRMpQKM1MVKaHCOmqkKoDCNOXTHkUCOwzGCe9H2HrxZkkpm9PTDRAmomTFQaZgRwRpmDDrhs9HGQAzjeCXla8D4JznG/t+3oOy8HxxEhrQHrZYWogKp2Ia2YDzbiFRmH9qADuwjSeSDw3SGMwr6Pjq2QWb1kiJY9k8lmWICL8EZJpA8fFouPrY7TV/vfZ0I2rVdnKw1k+sE+aUkZ+6SGGVRCN7mvOA4OAmjRSpkYcqDfcpdkBAwT/JjstIk6upsj7ox54ByEvIgSt5cLDowyOFzYONTtGkDOdtIAhRToIYQmYICq12OWu5SaUj3YkkTRvLI/gJSRMH83sEfiJHgcalMPZRRTKS7K0s5uvENtGa13/Wu1mvc8NXfd4cDvxOpN38aNuMjUv8C);strokeColor=none;spacingTop=-3;spacingBottom=-3;spacingLeft=-3;spacingRight=-3;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-405" vertex="1">
          <mxGeometry x="13" y="5" width="16" height="22" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-408" style="vsdxID=354;rotation=60;fillColor=#FFFFFF;gradientColor=none;shape=stencil(fVTtboMwDHwVlAdwkzifEvAu1UoHWtdOlG7t28/BoYXS7Z/lA99dfEl5brdfTXEe+tNH89PthrYS3bFt+m4Qdbk/9c17f7ocd3X5tR3auvw8fTfFtRLWgtSiuFVCgrRiU5dvlz5BqhKoIEEqY8VVV0JRidRMpQKM1MVKaHCOmqkKoDCNOXTHkUCOwzGCe9H2HrxZkkpm9PTDRAmomTFQaZgRwRpmDDrhs9HGQAzjeCXla8D4JznG/t+3oOy8HxxEhrQHrZYWogKp2Ia2YDzbiFRmH9qADuwjSeSDw3SGMwr6Pjq2QWb1kiJY9k8lmWICL8EZJpA8fFouPrY7TV/vfZ0I2rVdnKw1k+sE+aUkZ+6SGGVRCN7mvOA4OAmjRSpkYcqDfcpdkBAwT/JjstIk6upsj7ox54ByEvIgSt5cLDowyOFzYONTtGkDOdtIAhRToIYQmYICq12OWu5SaUj3YkkTRvLI/gJSRMH83sEfiJHgcalMPZRRTKS7K0s5uvENtGa13/Wu1mvc8NXfd4cDvxOpN38aNuMjUv8C);strokeColor=none;spacingTop=-3;spacingBottom=-3;spacingLeft=-3;spacingRight=-3;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-405" vertex="1">
          <mxGeometry x="20" y="7" width="16" height="22" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-409" style="vsdxID=355;rotation=120;fillColor=#FFFFFF;gradientColor=none;shape=stencil(fVTtboMwDHwVlAdwkzifEvAu1UoHWtdOlG7t28/BoYXS7Z/lA99dfEl5brdfTXEe+tNH89PthrYS3bFt+m4Qdbk/9c17f7ocd3X5tR3auvw8fTfFtRLWgtSiuFVCgrRiU5dvlz5BqhKoIEEqY8VVV0JRidRMpQKM1MVKaHCOmqkKoDCNOXTHkUCOwzGCe9H2HrxZkkpm9PTDRAmomTFQaZgRwRpmDDrhs9HGQAzjeCXla8D4JznG/t+3oOy8HxxEhrQHrZYWogKp2Ia2YDzbiFRmH9qADuwjSeSDw3SGMwr6Pjq2QWb1kiJY9k8lmWICL8EZJpA8fFouPrY7TV/vfZ0I2rVdnKw1k+sE+aUkZ+6SGGVRCN7mvOA4OAmjRSpkYcqDfcpdkBAwT/JjstIk6upsj7ox54ByEvIgSt5cLDowyOFzYONTtGkDOdtIAhRToIYQmYICq12OWu5SaUj3YkkTRvLI/gJSRMH83sEfiJHgcalMPZRRTKS7K0s5uvENtGa13/Wu1mvc8NXfd4cDvxOpN38aNuMjUv8C);strokeColor=none;spacingTop=-3;spacingBottom=-3;spacingLeft=-3;spacingRight=-3;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-405" vertex="1">
          <mxGeometry x="23" y="13" width="16" height="22" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-410" style="vsdxID=356;rotation=180;fillColor=#FFFFFF;gradientColor=none;shape=stencil(fVTtboMwDHwVlAdwkzifEvAu1UoHWtdOlG7t28/BoYXS7Z/lA99dfEl5brdfTXEe+tNH89PthrYS3bFt+m4Qdbk/9c17f7ocd3X5tR3auvw8fTfFtRLWgtSiuFVCgrRiU5dvlz5BqhKoIEEqY8VVV0JRidRMpQKM1MVKaHCOmqkKoDCNOXTHkUCOwzGCe9H2HrxZkkpm9PTDRAmomTFQaZgRwRpmDDrhs9HGQAzjeCXla8D4JznG/t+3oOy8HxxEhrQHrZYWogKp2Ia2YDzbiFRmH9qADuwjSeSDw3SGMwr6Pjq2QWb1kiJY9k8lmWICL8EZJpA8fFouPrY7TV/vfZ0I2rVdnKw1k+sE+aUkZ+6SGGVRCN7mvOA4OAmjRSpkYcqDfcpdkBAwT/JjstIk6upsj7ox54ByEvIgSt5cLDowyOFzYONTtGkDOdtIAhRToIYQmYICq12OWu5SaUj3YkkTRvLI/gJSRMH83sEfiJHgcalMPZRRTKS7K0s5uvENtGa13/Wu1mvc8NXfd4cDvxOpN38aNuMjUv8C);strokeColor=none;spacingTop=-3;spacingBottom=-3;spacingLeft=-3;spacingRight=-3;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-405" vertex="1">
          <mxGeometry x="18" y="19" width="16" height="22" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-411" style="vsdxID=357;rotation=240;fillColor=#FFFFFF;gradientColor=none;shape=stencil(fVTtboMwDHwVlAdwkzifEvAu1UoHWtdOlG7t28/BoYXS7Z/lA99dfEl5brdfTXEe+tNH89PthrYS3bFt+m4Qdbk/9c17f7ocd3X5tR3auvw8fTfFtRLWgtSiuFVCgrRiU5dvlz5BqhKoIEEqY8VVV0JRidRMpQKM1MVKaHCOmqkKoDCNOXTHkUCOwzGCe9H2HrxZkkpm9PTDRAmomTFQaZgRwRpmDDrhs9HGQAzjeCXla8D4JznG/t+3oOy8HxxEhrQHrZYWogKp2Ia2YDzbiFRmH9qADuwjSeSDw3SGMwr6Pjq2QWb1kiJY9k8lmWICL8EZJpA8fFouPrY7TV/vfZ0I2rVdnKw1k+sE+aUkZ+6SGGVRCN7mvOA4OAmjRSpkYcqDfcpdkBAwT/JjstIk6upsj7ox54ByEvIgSt5cLDowyOFzYONTtGkDOdtIAhRToIYQmYICq12OWu5SaUj3YkkTRvLI/gJSRMH83sEfiJHgcalMPZRRTKS7K0s5uvENtGa13/Wu1mvc8NXfd4cDvxOpN38aNuMjUv8C);strokeColor=none;spacingTop=-3;spacingBottom=-3;spacingLeft=-3;spacingRight=-3;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-405" vertex="1">
          <mxGeometry x="11" y="18" width="16" height="22" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-412" style="vsdxID=358;rotation=300;fillColor=#FFFFFF;gradientColor=none;shape=stencil(fVTtboMwDHwVlAdwkzifEvAu1UoHWtdOlG7t28/BoYXS7Z/lA99dfEl5brdfTXEe+tNH89PthrYS3bFt+m4Qdbk/9c17f7ocd3X5tR3auvw8fTfFtRLWgtSiuFVCgrRiU5dvlz5BqhKoIEEqY8VVV0JRidRMpQKM1MVKaHCOmqkKoDCNOXTHkUCOwzGCe9H2HrxZkkpm9PTDRAmomTFQaZgRwRpmDDrhs9HGQAzjeCXla8D4JznG/t+3oOy8HxxEhrQHrZYWogKp2Ia2YDzbiFRmH9qADuwjSeSDw3SGMwr6Pjq2QWb1kiJY9k8lmWICL8EZJpA8fFouPrY7TV/vfZ0I2rVdnKw1k+sE+aUkZ+6SGGVRCN7mvOA4OAmjRSpkYcqDfcpdkBAwT/JjstIk6upsj7ox54ByEvIgSt5cLDowyOFzYONTtGkDOdtIAhRToIYQmYICq12OWu5SaUj3YkkTRvLI/gJSRMH83sEfiJHgcalMPZRRTKS7K0s5uvENtGa13/Wu1mvc8NXfd4cDvxOpN38aNuMjUv8C);strokeColor=none;spacingTop=-3;spacingBottom=-3;spacingLeft=-3;spacingRight=-3;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-405" vertex="1">
          <mxGeometry x="8" y="11" width="16" height="22" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-299" value="&lt;font style=&quot;font-size: 18px;&quot; face=&quot;Calibri&quot;&gt;&lt;b style=&quot;&quot;&gt;Filter&lt;/b&gt;&lt;/font&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#FFF4FE;strokeColor=#9673a6;" parent="1" vertex="1">
          <mxGeometry x="-1475" y="289" width="55" height="64" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-302" style="vsdxID=751;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeWidth=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.999;exitY=0.501;exitDx=0;exitDy=0;exitPerimeter=0;" parent="1" source="ZVaZIW3ceO06EkHoMhZQ-437" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="-1398" y="321.34" as="sourcePoint" />
            <mxPoint x="-1310" y="321" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-693" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\mathcal{V}^{k-1}$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" parent="1" vertex="1">
          <mxGeometry x="-1801" y="482.5" width="200" height="40" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-335" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="-1633" y="444" width="999" height="210" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-491" value="" style="verticalAlign=middle;align=center;vsdxID=280;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLbjsIgFPwVct6hF60rCeVfiKUtWbY0p6j1761gFX3ZTdwnwgyZGc4ZMfVq1GTy6L712TS+r8EMvUbjQYrWoe7QHYdGilH5Xoofd9JkrqHIgVxuRw6ZFNYMAeV/QBUeCAYFVmyAYGDYDqJqfLrnrFq4marZTBSdV964oYaFtQo7TRcR2lrVBWg6az0+ronxKrfob79Sb87KMlpztqsgCUnzz22fUi9ZfgOf4ao1G4/Z0l98nC6d8Os69veZFAXblPC25X9YRtqCLNapNdbG7t2wtG5ZKKa8Ag==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-335" vertex="1">
          <mxGeometry x="64" y="37.5" width="106" height="101" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-686" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\mathcal{T}^{k}$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" parent="nIato8iqnGkG7OKb6TYW-335" vertex="1">
          <mxGeometry y="37.5" width="180" height="40" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-317" value="" style="group" parent="nIato8iqnGkG7OKb6TYW-335" vertex="1" connectable="0">
          <mxGeometry x="101" y="78.5" width="220" height="58" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-304" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:top;direction:ltr;&quot;&gt;&lt;br&gt;&lt;/p&gt;" style="verticalAlign=top;align=center;vsdxID=432;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLbjsIgFPwVct6hF22VhPIvRGlLZEtzym71763gBX0wJu4TYQ6ZmcOMmHo1ajJ5dAc9m73vGzBDr9F4kKJ1qDt0v8NeilH5Xoof96fJsYEiB3K6HDlkUlgzBJR/gCrcEQwMrKiBYJiweg2RNr7dclatFoSqo5koOq+8cUMDy9Qq7DRdWGhrVRegadZ6vF8T5RvdIrDepOKclWXU5qyuIHFJ8+9lr1QvVt5jD2fVzRiPxtIVvraWfu9zGJvtNYyClRxeMv6HJNIOZLFMrbE2Nu+CpWXLQi3lGQ==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-317" vertex="1">
          <mxGeometry x="83" y="2" width="106" height="58" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-305" style="vsdxID=320;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-317" vertex="1">
          <mxGeometry x="130.5" y="39.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-306" style="vsdxID=323;fillColor=#f7cbac;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-317" vertex="1">
          <mxGeometry x="101" y="40" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-307" style="vsdxID=322;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-317" vertex="1">
          <mxGeometry x="159" y="40" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-308" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\mathcal{V}_{sel}^k$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" parent="nIato8iqnGkG7OKb6TYW-317" vertex="1">
          <mxGeometry width="220" height="40" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-652" style="vsdxID=479;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);dashed=1;strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-335" vertex="1">
          <mxGeometry x="54" y="2" width="239" height="144.5" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-492" style="vsdxID=281;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-335" vertex="1">
          <mxGeometry x="114" y="65.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-493" style="vsdxID=282;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-335" vertex="1">
          <mxGeometry x="91" y="94.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-494" style="vsdxID=283;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-335" vertex="1">
          <mxGeometry x="136" y="94.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-495" style="vsdxID=286;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-335" vertex="1">
          <mxGeometry x="78" y="120.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-496" style="vsdxID=287;fillColor=#f7cbac;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-335" vertex="1">
          <mxGeometry x="105" y="120.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-497" style="vsdxID=288;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-335" vertex="1">
          <mxGeometry x="136" y="120.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-498" style="vsdxID=284;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.15384615384615385;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.5384615384615384;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="nIato8iqnGkG7OKb6TYW-335" source="ZVaZIW3ceO06EkHoMhZQ-492" target="ZVaZIW3ceO06EkHoMhZQ-493" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="683" y="552.5" as="sourcePoint" />
            <mxPoint x="665" y="570.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-4" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-499" style="vsdxID=285;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.8461538461538461;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.46153846153846156;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="nIato8iqnGkG7OKb6TYW-335" source="ZVaZIW3ceO06EkHoMhZQ-492" target="ZVaZIW3ceO06EkHoMhZQ-494" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="692" y="552.5" as="sourcePoint" />
            <mxPoint x="709" y="570.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="4" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-500" value="" style="vsdxID=289;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;align=center;exitX=0.15384615384615385;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.5384615384615384;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="nIato8iqnGkG7OKb6TYW-335" source="ZVaZIW3ceO06EkHoMhZQ-493" target="ZVaZIW3ceO06EkHoMhZQ-495" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="660" y="581.5" as="sourcePoint" />
            <mxPoint x="652" y="596.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-9" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-501" style="vsdxID=290;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.9230769230769231;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.46153846153846156;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="nIato8iqnGkG7OKb6TYW-335" source="ZVaZIW3ceO06EkHoMhZQ-493" target="ZVaZIW3ceO06EkHoMhZQ-496" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="670" y="581.5" as="sourcePoint" />
            <mxPoint x="678" y="596.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="8" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-502" style="vsdxID=291;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.46153846153846156;exitY=1;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.46153846153846156;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="nIato8iqnGkG7OKb6TYW-335" source="ZVaZIW3ceO06EkHoMhZQ-494" target="ZVaZIW3ceO06EkHoMhZQ-497" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="709" y="583.5" as="sourcePoint" />
            <mxPoint x="709" y="596.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-13" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-318" value="" style="group" parent="nIato8iqnGkG7OKb6TYW-335" vertex="1" connectable="0">
          <mxGeometry x="119" y="20" width="880" height="190" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-536" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:top;direction:ltr;&quot;&gt;&lt;br&gt;&lt;/p&gt;" style="verticalAlign=top;align=center;vsdxID=432;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLbjsIgFPwVct6hF22VhPIvRGlLZEtzym71763gBX0wJu4TYQ6ZmcOMmHo1ajJ5dAc9m73vGzBDr9F4kKJ1qDt0v8NeilH5Xoof96fJsYEiB3K6HDlkUlgzBJR/gCrcEQwMrKiBYJiweg2RNr7dclatFoSqo5koOq+8cUMDy9Qq7DRdWGhrVRegadZ6vF8T5RvdIrDepOKclWXU5qyuIHFJ8+9lr1QvVt5jD2fVzRiPxtIVvraWfu9zGJvtNYyClRxeMv6HJNIOZLFMrbE2Nu+CpWXLQi3lGQ==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-318" vertex="1">
          <mxGeometry x="64" y="2" width="106" height="58" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-740" style="vsdxID=286;fillColor=#BDD7EE;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-318" vertex="1">
          <mxGeometry x="110.5" y="39.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-741" style="vsdxID=286;fillColor=#BDD7EE;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-318" vertex="1">
          <mxGeometry x="81" y="39" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-742" style="vsdxID=286;fillColor=#BDD7EE;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-318" vertex="1">
          <mxGeometry x="139" y="38.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-743" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\mathcal{V}^k$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" parent="nIato8iqnGkG7OKb6TYW-318" vertex="1">
          <mxGeometry y="2" width="170" height="40" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-315" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$M_2$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" vertex="1" parent="nIato8iqnGkG7OKb6TYW-318">
          <mxGeometry x="224" y="-24" width="100" height="40" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-310" value="&lt;b style=&quot;border-color: var(--border-color); color: rgb(0, 0, 0); font-family: Calibri; font-style: normal; font-variant-ligatures: normal; font-variant-caps: normal; letter-spacing: normal; orphans: 2; text-indent: 0px; text-transform: none; widows: 2; word-spacing: 0px; -webkit-text-stroke-width: 0px; text-decoration-thickness: initial; text-decoration-style: initial; text-decoration-color: initial;&quot;&gt;&lt;font style=&quot;font-size: 18px;&quot;&gt;CoL-K Output&lt;/font&gt;&lt;/b&gt;" style="text;whiteSpace=wrap;html=1;align=left;fillColor=none;" parent="nIato8iqnGkG7OKb6TYW-335" vertex="1">
          <mxGeometry x="54" y="2" width="120" height="30" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-350" value="&lt;font style=&quot;font-size: 18px;&quot; face=&quot;Calibri&quot;&gt;&lt;b style=&quot;&quot;&gt;CoL-K&lt;/b&gt;&lt;/font&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#dae8fc;strokeColor=#6c8ebf;" parent="1" vertex="1">
          <mxGeometry x="-1548.32" y="290" width="58.32" height="63" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-357" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="-935" y="444" width="238" height="144.5" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-401" style="vsdxID=480;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);dashed=1;strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-357" vertex="1">
          <mxGeometry x="1" width="238" height="144.5" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-390" value="" style="verticalAlign=middle;align=center;vsdxID=441;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLbjsIgFPwVct6hF60rCeVfiKUtWbY0p6j1761gFX3ZTdwnwgyZGc4ZMfVq1GTy6L712TS+r8EMvUbjQYrWoe7QHYdGilH5Xoofd9JkrqHIgVxuRw6ZFNYMAeV/QBUeCAYFVmyAYGDYDqJqfLrnrFq4marZTBSdV964oYaFtQo7TRcR2lrVBWg6az0+ronxKrfob79Sb87KMlpztqsgCUnzz22fUi9ZfgOf4ao1G4/Z0l98nC6d8Os69veZFAXblPC25X9YRtqCLNapNdbG7t2wtG5ZKKa8Ag==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-357" vertex="1">
          <mxGeometry x="8" y="34.5" width="106" height="101" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-391" style="vsdxID=442;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-357" vertex="1">
          <mxGeometry x="58" y="61.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-392" style="vsdxID=443;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-357" vertex="1">
          <mxGeometry x="36" y="90.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-393" style="vsdxID=444;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-357" vertex="1">
          <mxGeometry x="80" y="90.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-394" style="vsdxID=447;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-357" vertex="1">
          <mxGeometry x="36" y="117.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-395" style="vsdxID=449;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-357" vertex="1">
          <mxGeometry x="80" y="117.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-559" style="vsdxID=452;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.5384615384615384;exitY=1;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.5384615384615384;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="nIato8iqnGkG7OKb6TYW-357" source="ZVaZIW3ceO06EkHoMhZQ-393" target="ZVaZIW3ceO06EkHoMhZQ-395" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="87" y="103.5" as="sourcePoint" />
            <mxPoint x="87" y="117.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-13" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-560" value="" style="vsdxID=450;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;align=center;exitX=0.46153846153846156;exitY=1;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.46153846153846156;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="nIato8iqnGkG7OKb6TYW-357" source="ZVaZIW3ceO06EkHoMhZQ-392" target="ZVaZIW3ceO06EkHoMhZQ-394" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="42" y="103.5" as="sourcePoint" />
            <mxPoint x="42" y="117.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="12" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-561" style="vsdxID=446;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.8461538461538461;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.5384615384615384;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="nIato8iqnGkG7OKb6TYW-357" source="ZVaZIW3ceO06EkHoMhZQ-391" target="ZVaZIW3ceO06EkHoMhZQ-393" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="69" y="72.5" as="sourcePoint" />
            <mxPoint x="87" y="90.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="4" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-562" style="vsdxID=445;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.15384615384615385;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.46153846153846156;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="nIato8iqnGkG7OKb6TYW-357" source="ZVaZIW3ceO06EkHoMhZQ-391" target="ZVaZIW3ceO06EkHoMhZQ-392" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="60" y="72.5" as="sourcePoint" />
            <mxPoint x="42" y="90.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-4" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-763" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:top;direction:ltr;&quot;&gt;&lt;br&gt;&lt;/p&gt;" style="verticalAlign=top;align=center;vsdxID=432;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLbjsIgFPwVct6hF22VhPIvRGlLZEtzym71763gBX0wJu4TYQ6ZmcOMmHo1ajJ5dAc9m73vGzBDr9F4kKJ1qDt0v8NeilH5Xoof96fJsYEiB3K6HDlkUlgzBJR/gCrcEQwMrKiBYJiweg2RNr7dclatFoSqo5koOq+8cUMDy9Qq7DRdWGhrVRegadZ6vF8T5RvdIrDepOKclWXU5qyuIHFJ8+9lr1QvVt5jD2fVzRiPxtIVvraWfu9zGJvtNYyClRxeMv6HJNIOZLFMrbE2Nu+CpWXLQi3lGQ==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-357" vertex="1">
          <mxGeometry x="126" y="34.5" width="106" height="101" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-764" style="vsdxID=286;fillColor=#BDD7EE;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-357" vertex="1">
          <mxGeometry x="189" y="99.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-765" style="vsdxID=286;fillColor=#BDD7EE;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-357" vertex="1">
          <mxGeometry x="155" y="99.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-766" style="vsdxID=286;fillColor=#BDD7EE;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-357" vertex="1">
          <mxGeometry x="189" y="74.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-767" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\mathcal{V}^k$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" parent="nIato8iqnGkG7OKb6TYW-357" vertex="1">
          <mxGeometry x="62" y="34.5" width="170" height="40" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-768" style="vsdxID=287;fillColor=#f7cbac;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-357" vertex="1">
          <mxGeometry x="155" y="74" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-333" value="&lt;b style=&quot;border-color: var(--border-color); color: rgb(0, 0, 0); font-family: Calibri; font-style: normal; font-variant-ligatures: normal; font-variant-caps: normal; letter-spacing: normal; orphans: 2; text-indent: 0px; text-transform: none; widows: 2; word-spacing: 0px; -webkit-text-stroke-width: 0px; text-decoration-thickness: initial; text-decoration-style: initial; text-decoration-color: initial;&quot;&gt;&lt;font style=&quot;font-size: 18px;&quot;&gt;Filter Output&lt;/font&gt;&lt;/b&gt;" style="text;whiteSpace=wrap;html=1;align=left;labelBackgroundColor=none;" parent="nIato8iqnGkG7OKb6TYW-357" vertex="1">
          <mxGeometry x="2" y="1" width="120" height="30" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-287" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\mathcal{T}^{k}$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" vertex="1" parent="nIato8iqnGkG7OKb6TYW-357">
          <mxGeometry x="-59" y="34.5" width="180" height="40" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-369" style="vsdxID=751;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeWidth=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;entryX=0;entryY=0.557;entryDx=0;entryDy=0;entryPerimeter=0;exitX=1.001;exitY=0.548;exitDx=0;exitDy=0;exitPerimeter=0;" parent="1" target="ZVaZIW3ceO06EkHoMhZQ-314" edge="1" source="ZVaZIW3ceO06EkHoMhZQ-652">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="-1350" y="524" as="sourcePoint" />
            <mxPoint x="-1265" y="524.36" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-370" style="vsdxID=751;edgeStyle=orthogonalEdgeStyle;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeWidth=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.258;exitY=1.004;exitDx=0;exitDy=0;entryX=0;entryY=0.5;entryDx=0;entryDy=0;exitPerimeter=0;" parent="1" source="ZVaZIW3ceO06EkHoMhZQ-656" target="ZVaZIW3ceO06EkHoMhZQ-786" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="-1364" y="536.36" as="sourcePoint" />
            <mxPoint x="-1276" y="536" as="targetPoint" />
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-371" style="vsdxID=751;edgeStyle=orthogonalEdgeStyle;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeWidth=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=1;exitY=0.5;exitDx=0;exitDy=0;entryX=0.759;entryY=1.009;entryDx=0;entryDy=0;entryPerimeter=0;" parent="1" source="ZVaZIW3ceO06EkHoMhZQ-786" target="ZVaZIW3ceO06EkHoMhZQ-652" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="-1790" y="602" as="sourcePoint" />
            <mxPoint x="-1706" y="638" as="targetPoint" />
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-372" value="" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#FFF4FE;strokeColor=#9673a6;labelBorderColor=#000000;" parent="1" vertex="1">
          <mxGeometry x="-963.02" y="597.88" width="170" height="55.82" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-382" value="&lt;p style=&quot;border-color: var(--border-color); color: rgb(0, 0, 0); font-style: normal; font-variant-ligatures: normal; font-variant-caps: normal; font-weight: 400; letter-spacing: normal; orphans: 2; text-align: center; text-indent: 0px; text-transform: none; widows: 2; word-spacing: 0px; -webkit-text-stroke-width: 0px; text-decoration-thickness: initial; text-decoration-style: initial; text-decoration-color: initial; margin: 0px; direction: ltr;&quot;&gt;&lt;font face=&quot;Calibri&quot; style=&quot;font-size: 18px;&quot;&gt;&lt;font style=&quot;border-color: var(--border-color); letter-spacing: 0px; direction: ltr; line-height: 28.8px; opacity: 1;&quot;&gt;&lt;b style=&quot;border-color: var(--border-color);&quot;&gt;Filter&lt;/b&gt;&lt;/font&gt;&lt;font style=&quot;border-color: var(--border-color); letter-spacing: 0px; direction: ltr; line-height: 14.4px; opacity: 1;&quot;&gt;&lt;b style=&quot;border-color: var(--border-color);&quot;&gt;&lt;font style=&quot;border-color: var(--border-color);&quot;&gt;&amp;nbsp;out the&lt;/font&gt;&lt;/b&gt;&lt;/font&gt;&lt;/font&gt;&lt;/p&gt;&lt;p style=&quot;border-color: var(--border-color); color: rgb(0, 0, 0); font-style: normal; font-variant-ligatures: normal; font-variant-caps: normal; font-weight: 400; letter-spacing: normal; orphans: 2; text-align: center; text-indent: 0px; text-transform: none; widows: 2; word-spacing: 0px; -webkit-text-stroke-width: 0px; text-decoration-thickness: initial; text-decoration-style: initial; text-decoration-color: initial; margin: 0px; direction: ltr;&quot;&gt;&lt;b style=&quot;letter-spacing: 0px; font-size: 18px; font-family: Calibri; background-color: initial; border-color: var(--border-color);&quot;&gt;&lt;font style=&quot;border-color: var(--border-color);&quot;&gt;hallucination&lt;/font&gt;&lt;/b&gt;&lt;/p&gt;" style="text;whiteSpace=wrap;html=1;" parent="1" vertex="1">
          <mxGeometry x="-930" y="593" width="113" height="70" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-383" style="vsdxID=751;edgeStyle=orthogonalEdgeStyle;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeWidth=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.281;exitY=1.002;exitDx=0;exitDy=0;entryX=0;entryY=0.5;entryDx=0;entryDy=0;exitPerimeter=0;" parent="1" source="ZVaZIW3ceO06EkHoMhZQ-314" target="nIato8iqnGkG7OKb6TYW-372" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="-1795" y="600" as="sourcePoint" />
            <mxPoint x="-1704" y="636" as="targetPoint" />
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-384" style="vsdxID=751;edgeStyle=orthogonalEdgeStyle;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeWidth=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=1;exitY=0.5;exitDx=0;exitDy=0;entryX=0.76;entryY=1.002;entryDx=0;entryDy=0;entryPerimeter=0;" parent="1" source="nIato8iqnGkG7OKb6TYW-372" target="ZVaZIW3ceO06EkHoMhZQ-401" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="-1214" y="599" as="sourcePoint" />
            <mxPoint x="-1068" y="636" as="targetPoint" />
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-288" value="&lt;i style=&quot;border-color: var(--border-color); color: rgb(0, 0, 0); font-family: Calibri; font-variant-ligatures: normal; font-variant-caps: normal; font-weight: 400; letter-spacing: normal; orphans: 2; text-align: left; text-indent: 0px; text-transform: none; widows: 2; word-spacing: 0px; -webkit-text-stroke-width: 0px; text-decoration-thickness: initial; text-decoration-style: initial; text-decoration-color: initial;&quot;&gt;&lt;b style=&quot;border-color: var(--border-color);&quot;&gt;&lt;font style=&quot;font-size: 18px;&quot;&gt;1. science&lt;br style=&quot;border-color: var(--border-color);&quot;&gt;1.1 physics&lt;br style=&quot;border-color: var(--border-color);&quot;&gt;...&lt;br style=&quot;border-color: var(--border-color);&quot;&gt;1.2 chemistry&lt;br style=&quot;border-color: var(--border-color);&quot;&gt;...&lt;/font&gt;&lt;/b&gt;&lt;/i&gt;" style="text;whiteSpace=wrap;html=1;labelBackgroundColor=none;" vertex="1" parent="1">
          <mxGeometry x="-999" y="257.25" width="130" height="124.5" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-453" style="vsdxID=271;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLRDoIgFP0Vdt9BLSvZkH9hhcoicVcq+/tUZlEvtdUT41x2zuGeI/pGdZr0Ht1RX83BNyWYttFoPEhROdQ1unN7kKJTvpHi5C6aDCVkKZDbdKSQSGFNO6P8C1ThnuDMwLZAcBwUjEPgDA95Nk0GqgbTU3ReeePaEsahVVhrOjLQyqp6hvqr1t3jGqkubAXLY9mCFZsgu2P5GiJ/NP1d9En14uQTuJjjLM8Wc2Enzz/87C1a7msMa77ksFvBW7h/iCEOPwktqoy1oXITFrcsmfso7w==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="-840.5" y="251.5" width="133" height="128" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-307" value="" style="group" vertex="1" connectable="0" parent="1">
          <mxGeometry x="-840.5" y="251.5" width="133" height="128" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-290" style="vsdxID=271;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLRDoIgFP0Vdt9BLSvZkH9hhcoicVcq+/tUZlEvtdUT41x2zuGeI/pGdZr0Ht1RX83BNyWYttFoPEhROdQ1unN7kKJTvpHi5C6aDCVkKZDbdKSQSGFNO6P8C1ThnuDMwLZAcBwUjEPgDA95Nk0GqgbTU3ReeePaEsahVVhrOjLQyqp6hvqr1t3jGqkubAXLY9mCFZsgu2P5GiJ/NP1d9En14uQTuJjjLM8Wc2Enzz/87C1a7msMa77ksFvBW7h/iCEOPwktqoy1oXITFrcsmfso7w==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" vertex="1" parent="RbdjuNJBBSJslo0sPhe3-307">
          <mxGeometry width="133" height="128" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-289" style="vsdxID=447;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" vertex="1" parent="RbdjuNJBBSJslo0sPhe3-307">
          <mxGeometry x="60.75" y="7" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-291" style="vsdxID=447;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" vertex="1" parent="RbdjuNJBBSJslo0sPhe3-307">
          <mxGeometry x="31.25" y="30" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-292" style="vsdxID=447;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" vertex="1" parent="RbdjuNJBBSJslo0sPhe3-307">
          <mxGeometry x="89.79999999999995" y="30" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-293" style="vsdxID=447;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" vertex="1" parent="RbdjuNJBBSJslo0sPhe3-307">
          <mxGeometry x="31.25" y="66" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-294" style="vsdxID=447;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" vertex="1" parent="RbdjuNJBBSJslo0sPhe3-307">
          <mxGeometry x="89.79999999999995" y="66" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-295" style="vsdxID=447;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" vertex="1" parent="RbdjuNJBBSJslo0sPhe3-307">
          <mxGeometry x="12.75" y="96" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-296" style="vsdxID=447;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" vertex="1" parent="RbdjuNJBBSJslo0sPhe3-307">
          <mxGeometry x="47.75" y="96" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-297" style="vsdxID=447;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" vertex="1" parent="RbdjuNJBBSJslo0sPhe3-307">
          <mxGeometry x="73.79999999999995" y="96" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-298" style="vsdxID=447;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" vertex="1" parent="RbdjuNJBBSJslo0sPhe3-307">
          <mxGeometry x="106.79999999999995" y="96" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-299" style="vsdxID=364;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;entryX=0.568;entryY=-0.033;entryDx=0;entryDy=0;entryPerimeter=0;exitX=0.505;exitY=0.996;exitDx=0;exitDy=0;exitPerimeter=0;" edge="1" parent="RbdjuNJBBSJslo0sPhe3-307" source="RbdjuNJBBSJslo0sPhe3-289" target="RbdjuNJBBSJslo0sPhe3-291">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="-94.20000000000005" y="39" as="sourcePoint" />
            <mxPoint x="-120.20000000000005" y="53" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-2" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-300" style="vsdxID=364;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;entryX=0.5;entryY=-0.01;entryDx=0;entryDy=0;entryPerimeter=0;" edge="1" parent="RbdjuNJBBSJslo0sPhe3-307" target="RbdjuNJBBSJslo0sPhe3-292">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="66.79999999999995" y="20" as="sourcePoint" />
            <mxPoint x="48.799999999999955" y="40" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-2" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-301" style="vsdxID=364;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;entryX=0.46;entryY=-0.048;entryDx=0;entryDy=0;entryPerimeter=0;exitX=0.472;exitY=1.028;exitDx=0;exitDy=0;exitPerimeter=0;" edge="1" parent="RbdjuNJBBSJslo0sPhe3-307" source="RbdjuNJBBSJslo0sPhe3-291" target="RbdjuNJBBSJslo0sPhe3-293">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="77.79999999999995" y="30" as="sourcePoint" />
            <mxPoint x="48.799999999999955" y="40" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-2" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-302" style="vsdxID=364;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;entryX=0.524;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0;exitX=0.5;exitY=1.052;exitDx=0;exitDy=0;exitPerimeter=0;" edge="1" parent="RbdjuNJBBSJslo0sPhe3-307" source="RbdjuNJBBSJslo0sPhe3-292" target="RbdjuNJBBSJslo0sPhe3-294">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="47.799999999999955" y="53" as="sourcePoint" />
            <mxPoint x="46.799999999999955" y="75" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-2" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-303" style="vsdxID=364;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;entryX=0.548;entryY=-0.054;entryDx=0;entryDy=0;entryPerimeter=0;exitX=0.496;exitY=1.002;exitDx=0;exitDy=0;exitPerimeter=0;" edge="1" parent="RbdjuNJBBSJslo0sPhe3-307" source="RbdjuNJBBSJslo0sPhe3-293" target="RbdjuNJBBSJslo0sPhe3-295">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="57.799999999999955" y="63" as="sourcePoint" />
            <mxPoint x="56.799999999999955" y="85" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-2" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-304" style="vsdxID=364;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;entryX=0.491;entryY=-0.03;entryDx=0;entryDy=0;entryPerimeter=0;exitX=0.508;exitY=1.014;exitDx=0;exitDy=0;exitPerimeter=0;" edge="1" parent="RbdjuNJBBSJslo0sPhe3-307" source="RbdjuNJBBSJslo0sPhe3-293" target="RbdjuNJBBSJslo0sPhe3-296">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="36.799999999999955" y="80" as="sourcePoint" />
            <mxPoint x="29.799999999999955" y="105" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-2" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-305" style="vsdxID=364;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;entryX=0.546;entryY=-0.054;entryDx=0;entryDy=0;entryPerimeter=0;exitX=0.493;exitY=1.01;exitDx=0;exitDy=0;exitPerimeter=0;" edge="1" parent="RbdjuNJBBSJslo0sPhe3-307" source="RbdjuNJBBSJslo0sPhe3-294" target="RbdjuNJBBSJslo0sPhe3-297">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="96.79999999999995" y="80" as="sourcePoint" />
            <mxPoint x="39.799999999999955" y="115" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-2" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-306" style="vsdxID=364;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;entryX=0.5;entryY=-0.038;entryDx=0;entryDy=0;entryPerimeter=0;exitX=0.491;exitY=1.026;exitDx=0;exitDy=0;exitPerimeter=0;" edge="1" parent="RbdjuNJBBSJslo0sPhe3-307" source="RbdjuNJBBSJslo0sPhe3-294" target="RbdjuNJBBSJslo0sPhe3-298">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="96.79999999999995" y="80" as="sourcePoint" />
            <mxPoint x="90.79999999999995" y="105" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-2" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-309" value="" style="group" vertex="1" connectable="0" parent="1">
          <mxGeometry x="-1270" y="444" width="320" height="144.5" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-320" value="" style="group" parent="RbdjuNJBBSJslo0sPhe3-309" vertex="1" connectable="0">
          <mxGeometry x="95" y="78.5" width="220" height="58" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-321" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:top;direction:ltr;&quot;&gt;&lt;br&gt;&lt;/p&gt;" style="verticalAlign=top;align=center;vsdxID=432;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLbjsIgFPwVct6hF22VhPIvRGlLZEtzym71763gBX0wJu4TYQ6ZmcOMmHo1ajJ5dAc9m73vGzBDr9F4kKJ1qDt0v8NeilH5Xoof96fJsYEiB3K6HDlkUlgzBJR/gCrcEQwMrKiBYJiweg2RNr7dclatFoSqo5koOq+8cUMDy9Qq7DRdWGhrVRegadZ6vF8T5RvdIrDepOKclWXU5qyuIHFJ8+9lr1QvVt5jD2fVzRiPxtIVvraWfu9zGJvtNYyClRxeMv6HJNIOZLFMrbE2Nu+CpWXLQi3lGQ==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-320" vertex="1">
          <mxGeometry x="83" width="106" height="58" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-322" style="vsdxID=320;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-320" vertex="1">
          <mxGeometry x="130.5" y="37.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-323" style="vsdxID=323;fillColor=#f7cbac;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-320" vertex="1">
          <mxGeometry x="101" y="38" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-324" style="vsdxID=322;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-320" vertex="1">
          <mxGeometry x="159" y="38" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-325" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\mathcal{V}_{sel}^k$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" parent="nIato8iqnGkG7OKb6TYW-320" vertex="1">
          <mxGeometry width="220" height="40" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-314" style="vsdxID=479;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);dashed=1;strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-309" vertex="1">
          <mxGeometry x="56" width="238" height="144.5" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-383" value="" style="verticalAlign=middle;align=center;vsdxID=416;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLbjsIgFPwVct6hF60rCeVfiKUtWbY0p6j1761gFX3ZTdwnwgyZGc4ZMfVq1GTy6L712TS+r8EMvUbjQYrWoe7QHYdGilH5Xoofd9JkrqHIgVxuRw6ZFNYMAeV/QBUeCAYFVmyAYGDYDqJqfLrnrFq4marZTBSdV964oYaFtQo7TRcR2lrVBWg6az0+ronxKrfob79Sb87KMlpztqsgCUnzz22fUi9ZfgOf4ao1G4/Z0l98nC6d8Os69veZFAXblPC25X9YRtqCLNapNdbG7t2wtG5ZKKa8Ag==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-309" vertex="1">
          <mxGeometry x="62" y="34.5" width="106" height="101" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-384" style="vsdxID=417;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-309" vertex="1">
          <mxGeometry x="112" y="61.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-385" style="vsdxID=418;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-309" vertex="1">
          <mxGeometry x="90" y="90.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-386" style="vsdxID=419;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-309" vertex="1">
          <mxGeometry x="134" y="90.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-387" style="vsdxID=422;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-309" vertex="1">
          <mxGeometry x="77" y="117.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-388" style="vsdxID=423;fillColor=#f7cbac;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-309" vertex="1">
          <mxGeometry x="103" y="117.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-389" style="vsdxID=424;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-309" vertex="1">
          <mxGeometry x="134" y="117.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-471" style="vsdxID=784;rotation=60;fillColor=none;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#ff0000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-309" vertex="1">
          <mxGeometry x="77" y="93.5" width="52" height="31" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-563" style="vsdxID=427;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.5384615384615384;exitY=1;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.5384615384615384;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="RbdjuNJBBSJslo0sPhe3-309" source="ZVaZIW3ceO06EkHoMhZQ-386" target="ZVaZIW3ceO06EkHoMhZQ-389" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="141" y="103.5" as="sourcePoint" />
            <mxPoint x="141" y="117.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-13" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-564" style="vsdxID=426;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.8461538461538461;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.5384615384615384;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="RbdjuNJBBSJslo0sPhe3-309" source="ZVaZIW3ceO06EkHoMhZQ-385" target="ZVaZIW3ceO06EkHoMhZQ-388" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="101" y="101.5" as="sourcePoint" />
            <mxPoint x="110" y="117.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="8" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-565" value="" style="vsdxID=425;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;align=center;exitX=0.15384615384615385;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.46153846153846156;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="RbdjuNJBBSJslo0sPhe3-309" source="ZVaZIW3ceO06EkHoMhZQ-385" target="ZVaZIW3ceO06EkHoMhZQ-387" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="92" y="101.5" as="sourcePoint" />
            <mxPoint x="83" y="117.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-9" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-570" style="vsdxID=420;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.15384615384615385;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.46153846153846156;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="RbdjuNJBBSJslo0sPhe3-309" source="ZVaZIW3ceO06EkHoMhZQ-384" target="ZVaZIW3ceO06EkHoMhZQ-385" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="114" y="72.5" as="sourcePoint" />
            <mxPoint x="96" y="90.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-4" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-571" style="vsdxID=421;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.8461538461538461;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.5384615384615384;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="RbdjuNJBBSJslo0sPhe3-309" source="ZVaZIW3ceO06EkHoMhZQ-384" target="ZVaZIW3ceO06EkHoMhZQ-386" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="123" y="72.5" as="sourcePoint" />
            <mxPoint x="141" y="90.5" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="4" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-326" value="" style="group" parent="RbdjuNJBBSJslo0sPhe3-309" vertex="1" connectable="0">
          <mxGeometry x="114" y="20" width="170" height="58" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-327" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:top;direction:ltr;&quot;&gt;&lt;br&gt;&lt;/p&gt;" style="verticalAlign=top;align=center;vsdxID=432;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLbjsIgFPwVct6hF22VhPIvRGlLZEtzym71763gBX0wJu4TYQ6ZmcOMmHo1ajJ5dAc9m73vGzBDr9F4kKJ1qDt0v8NeilH5Xoof96fJsYEiB3K6HDlkUlgzBJR/gCrcEQwMrKiBYJiweg2RNr7dclatFoSqo5koOq+8cUMDy9Qq7DRdWGhrVRegadZ6vF8T5RvdIrDepOKclWXU5qyuIHFJ8+9lr1QvVt5jD2fVzRiPxtIVvraWfu9zGJvtNYyClRxeMv6HJNIOZLFMrbE2Nu+CpWXLQi3lGQ==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-326" vertex="1">
          <mxGeometry x="64" width="106" height="58" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-328" style="vsdxID=286;fillColor=#BDD7EE;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-326" vertex="1">
          <mxGeometry x="110.5" y="37.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-329" style="vsdxID=286;fillColor=#BDD7EE;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-326" vertex="1">
          <mxGeometry x="81" y="37" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-330" style="vsdxID=286;fillColor=#BDD7EE;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="nIato8iqnGkG7OKb6TYW-326" vertex="1">
          <mxGeometry x="139" y="36.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-331" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\mathcal{V}^k$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" parent="nIato8iqnGkG7OKb6TYW-326" vertex="1">
          <mxGeometry width="170" height="40" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-332" value="&lt;b style=&quot;border-color: var(--border-color); color: rgb(0, 0, 0); font-family: Calibri; font-style: normal; font-variant-ligatures: normal; font-variant-caps: normal; letter-spacing: normal; orphans: 2; text-indent: 0px; text-transform: none; widows: 2; word-spacing: 0px; -webkit-text-stroke-width: 0px; text-decoration-thickness: initial; text-decoration-style: initial; text-decoration-color: initial;&quot;&gt;&lt;font style=&quot;font-size: 18px;&quot;&gt;Filter Input&lt;/font&gt;&lt;/b&gt;" style="text;whiteSpace=wrap;html=1;align=left;labelBackgroundColor=none;" parent="nIato8iqnGkG7OKb6TYW-326" vertex="1">
          <mxGeometry x="-56" y="-20" width="120" height="30" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-688" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\mathcal{T}^{k}$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" parent="RbdjuNJBBSJslo0sPhe3-309" vertex="1">
          <mxGeometry y="34.5" width="180" height="40" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-310" value="" style="group" vertex="1" connectable="0" parent="1">
          <mxGeometry x="-1899" y="446" width="288" height="144.5" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-489" value="" style="group" parent="RbdjuNJBBSJslo0sPhe3-310" connectable="0" vertex="1">
          <mxGeometry x="53" y="21.5" width="106" height="101" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-566" parent="RbdjuNJBBSJslo0sPhe3-310" vertex="1">
          <mxGeometry x="79.5" y="44.5" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-567" parent="RbdjuNJBBSJslo0sPhe3-310" vertex="1">
          <mxGeometry x="79.5" y="38.5" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-511" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:top;direction:ltr;&quot;&gt;&lt;br&gt;&lt;/p&gt;" style="verticalAlign=top;align=center;vsdxID=306;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLbjsIgFPwVct6hF22VhPIvRGlLZEtzym71763gBX0wJu4TYQ6ZmcOMmHo1ajJ5dAc9m73vGzBDr9F4kKJ1qDt0v8NeilH5Xoof96fJsYEiB3K6HDlkUlgzBJR/gCrcEQwMrKiBYJiweg2RNr7dclatFoSqo5koOq+8cUMDy9Qq7DRdWGhrVRegadZ6vF8T5RvdIrDepOKclWXU5qyuIHFJ8+9lr1QvVt5jD2fVzRiPxtIVvraWfu9zGJvtNYyClRxeMv6HJNIOZLFMrbE2Nu+CpWXLQi3lGQ==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-310" vertex="1">
          <mxGeometry x="174" y="35.5" width="106" height="101" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-656" style="vsdxID=479;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZDODTgv3YuJVRoRDOJv98bPQAc67Emad3F01cBqzCl2vEidnQUJjpNkIGxi4jbFKdSEQ5UdYR9nVqsFA2qzUBoDmtBLOPE4f7h46bfd7/pabMT7K++wZ5E+22kH);dashed=1;strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-310" vertex="1">
          <mxGeometry x="50" width="238" height="144.5" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-644" value="" style="group" parent="RbdjuNJBBSJslo0sPhe3-310" connectable="0" vertex="1">
          <mxGeometry x="59" y="35.5" width="106" height="101" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-504" style="vsdxID=274;fillColor=#fff2cc;gradientColor=none;shape=stencil(rVLbjsIgFPwVct6hF22VhPIvRGlLZEtzym71763gBX0wJu4TYQ6ZmcOMmHo1ajJ5dAc9m73vGzBDr9F4kKJ1qDt0v8NeilH5Xoof96fJsYEiB3K6HDlkUlgzBJR/gCrcEQwMrKiBYJiweg2RNr7dclatFoSqo5koOq+8cUMDy9Qq7DRdWGhrVRegadZ6vF8T5RvdIrDepOKclWXU5qyuIHFJ8+9lr1QvVt5jD2fVzRiPxtIVvraWfu9zGJvtNYyClRxeMv6HJNIOZLFMrbE2Nu+CpWXLQi3lGQ==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-644" vertex="1">
          <mxGeometry width="106" height="101" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-505" style="vsdxID=273;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-644" vertex="1">
          <mxGeometry x="47" y="34" width="13" height="12" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-506" style="vsdxID=276;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-644" vertex="1">
          <mxGeometry x="25" y="71" width="13" height="12" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-507" style="vsdxID=277;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-644" vertex="1">
          <mxGeometry x="69" y="71" width="13" height="12" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-508" style="vsdxID=278;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.15384615384615385;exitY=0.8333333333333334;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.46153846153846156;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="ZVaZIW3ceO06EkHoMhZQ-644" source="ZVaZIW3ceO06EkHoMhZQ-505" target="ZVaZIW3ceO06EkHoMhZQ-506" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="504" y="520" as="sourcePoint" />
            <mxPoint x="486" y="547" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-4" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-509" style="vsdxID=279;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.8461538461538461;exitY=0.8333333333333334;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.46153846153846156;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="ZVaZIW3ceO06EkHoMhZQ-644" source="ZVaZIW3ceO06EkHoMhZQ-505" target="ZVaZIW3ceO06EkHoMhZQ-507" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="513" y="520" as="sourcePoint" />
            <mxPoint x="530" y="547" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="4" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-687" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\mathcal{T}^{k-1}$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" parent="RbdjuNJBBSJslo0sPhe3-310" vertex="1">
          <mxGeometry y="35.5" width="200" height="40" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-724" style="vsdxID=286;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-310" vertex="1">
          <mxGeometry x="193" y="78.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-725" style="vsdxID=286;fillColor=#F7CBAC;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-310" vertex="1">
          <mxGeometry x="221" y="78.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-726" style="vsdxID=286;fillColor=#c5e0b3;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-310" vertex="1">
          <mxGeometry x="250" y="109" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-736" style="vsdxID=286;fillColor=#BDD7EE;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-310" vertex="1">
          <mxGeometry x="250" y="78.5" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-738" style="vsdxID=286;fillColor=#BDD7EE;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-310" vertex="1">
          <mxGeometry x="193" y="109" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-739" style="vsdxID=286;fillColor=#BDD7EE;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-310" vertex="1">
          <mxGeometry x="220.5" y="109" width="13" height="13" as="geometry" />
        </mxCell>
        <mxCell id="nIato8iqnGkG7OKb6TYW-309" value="&lt;b style=&quot;border-color: var(--border-color); color: rgb(0, 0, 0); font-family: Calibri; font-style: normal; font-variant-ligatures: normal; font-variant-caps: normal; letter-spacing: normal; orphans: 2; text-indent: 0px; text-transform: none; widows: 2; word-spacing: 0px; -webkit-text-stroke-width: 0px; text-decoration-thickness: initial; text-decoration-style: initial; text-decoration-color: initial;&quot;&gt;&lt;font style=&quot;font-size: 18px;&quot;&gt;CoL-K Input&lt;/font&gt;&lt;/b&gt;" style="text;whiteSpace=wrap;html=1;align=left;" parent="RbdjuNJBBSJslo0sPhe3-310" vertex="1">
          <mxGeometry x="49" width="120" height="30" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-314" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$M_1$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" vertex="1" parent="RbdjuNJBBSJslo0sPhe3-310">
          <mxGeometry x="-20.5" y="-5" width="100" height="40" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-311" value="" style="group" vertex="1" connectable="0" parent="1">
          <mxGeometry x="-1697" y="595.8807228915663" width="198.67669172932347" height="58.819277108433766" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-786" value="" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#dae8fc;strokeColor=#6c8ebf;labelBorderColor=#000000;" parent="RbdjuNJBBSJslo0sPhe3-311" vertex="1">
          <mxGeometry y="2.9992771084337164" width="170" height="55.82" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-668" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:top;direction:ltr;&quot;&gt;&lt;font face=&quot;Calibri&quot; style=&quot;color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1; font-size: 18px;&quot;&gt;&lt;b style=&quot;&quot;&gt;Select \(\mathcal{V}_{sel}^k\)&amp;nbsp;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:top;direction:ltr;&quot;&gt;&lt;font face=&quot;TbQWtvVfl1NGcp59eHHk&quot; style=&quot;color: rgb(0, 0, 0); direction: ltr; letter-spacing: 0px; line-height: 120%; opacity: 1; font-size: 18px;&quot;&gt;&lt;b style=&quot;&quot;&gt;Expand \(\mathcal{T}^{k-1}\)&lt;/b&gt;&lt;/font&gt;&lt;font style=&quot;font-size:25px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;&lt;br&gt;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=top;align=center;vsdxID=846;fillColor=none;gradientColor=none;shape=stencil(fc5LDoAgDEXRrZBuAJyX7sXEKo0IBvG3eyM60IEOe5LmXZxcPbKacoo9r9JkZ0GC4yQZCNuYuEtxDg3hWGdHOMSF1WbBgNotVMaAJvQSCp7nD7/wk+5nfe214v0Vd9qzR5dyOgA=);strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-311" vertex="1">
          <mxGeometry x="32.32330827067676" width="166.35338345864662" height="25.448275862068968" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-794" style="vsdxID=730;fillColor=none;gradientColor=none;strokeColor=none;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="RbdjuNJBBSJslo0sPhe3-311" vertex="1">
          <mxGeometry x="6" y="6.909277108433798" width="48" height="48" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-795" style="vsdxID=731;fillColor=#74aa9c;gradientColor=none;shape=stencil(dZFRDoMgEESvYjiAItSoCXIXU7GQWjWILd6+woqlTfq15E12djKwRbazSBajp7t4qc7IBqlRCq0M4qyftLjpaR07zubWSM4e01MktkEYJVuDyCXFOco4u67a8RyEfeQ4LQuUWHI+N+JFS2GN7IQ6sm8PavSmZZHWlTfG36ZVnZICjHEwxWAZDtHAaBQrGIMCM8Ihxyl8LobQ+bFsIb27eISxFAiF3HVs/NPOH5xBpb0aBujfsbjyzH8OfwM=);strokeColor=none;spacingTop=-3;spacingBottom=-3;spacingLeft=-3;spacingRight=-3;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-794" vertex="1">
          <mxGeometry width="48" height="48" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-796" style="vsdxID=732;fillColor=#FFFFFF;gradientColor=none;shape=stencil(fVTtboMwDHwVlAdwkzifEvAu1UoHWtdOlG7t28/BoYXS7Z/lA99dfEl5brdfTXEe+tNH89PthrYS3bFt+m4Qdbk/9c17f7ocd3X5tR3auvw8fTfFtRLWgtSiuFVCgrRiU5dvlz5BqhKoIEEqY8VVV0JRidRMpQKM1MVKaHCOmqkKoDCNOXTHkUCOwzGCe9H2HrxZkkpm9PTDRAmomTFQaZgRwRpmDDrhs9HGQAzjeCXla8D4JznG/t+3oOy8HxxEhrQHrZYWogKp2Ia2YDzbiFRmH9qADuwjSeSDw3SGMwr6Pjq2QWb1kiJY9k8lmWICL8EZJpA8fFouPrY7TV/vfZ0I2rVdnKw1k+sE+aUkZ+6SGGVRCN7mvOA4OAmjRSpkYcqDfcpdkBAwT/JjstIk6upsj7ox54ByEvIgSt5cLDowyOFzYONTtGkDOdtIAhRToIYQmYICq12OWu5SaUj3YkkTRvLI/gJSRMH83sEfiJHgcalMPZRRTKS7K0s5uvENtGa13/Wu1mvc8NXfd4cDvxOpN38aNuMjUv8C);strokeColor=none;spacingTop=-3;spacingBottom=-3;spacingLeft=-3;spacingRight=-3;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-794" vertex="1">
          <mxGeometry x="13" y="5" width="16" height="22" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-797" style="vsdxID=733;rotation=60;fillColor=#FFFFFF;gradientColor=none;shape=stencil(fVTtboMwDHwVlAdwkzifEvAu1UoHWtdOlG7t28/BoYXS7Z/lA99dfEl5brdfTXEe+tNH89PthrYS3bFt+m4Qdbk/9c17f7ocd3X5tR3auvw8fTfFtRLWgtSiuFVCgrRiU5dvlz5BqhKoIEEqY8VVV0JRidRMpQKM1MVKaHCOmqkKoDCNOXTHkUCOwzGCe9H2HrxZkkpm9PTDRAmomTFQaZgRwRpmDDrhs9HGQAzjeCXla8D4JznG/t+3oOy8HxxEhrQHrZYWogKp2Ia2YDzbiFRmH9qADuwjSeSDw3SGMwr6Pjq2QWb1kiJY9k8lmWICL8EZJpA8fFouPrY7TV/vfZ0I2rVdnKw1k+sE+aUkZ+6SGGVRCN7mvOA4OAmjRSpkYcqDfcpdkBAwT/JjstIk6upsj7ox54ByEvIgSt5cLDowyOFzYONTtGkDOdtIAhRToIYQmYICq12OWu5SaUj3YkkTRvLI/gJSRMH83sEfiJHgcalMPZRRTKS7K0s5uvENtGa13/Wu1mvc8NXfd4cDvxOpN38aNuMjUv8C);strokeColor=none;spacingTop=-3;spacingBottom=-3;spacingLeft=-3;spacingRight=-3;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-794" vertex="1">
          <mxGeometry x="20" y="7" width="16" height="22" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-798" style="vsdxID=734;rotation=120;fillColor=#FFFFFF;gradientColor=none;shape=stencil(fVTtboMwDHwVlAdwkzifEvAu1UoHWtdOlG7t28/BoYXS7Z/lA99dfEl5brdfTXEe+tNH89PthrYS3bFt+m4Qdbk/9c17f7ocd3X5tR3auvw8fTfFtRLWgtSiuFVCgrRiU5dvlz5BqhKoIEEqY8VVV0JRidRMpQKM1MVKaHCOmqkKoDCNOXTHkUCOwzGCe9H2HrxZkkpm9PTDRAmomTFQaZgRwRpmDDrhs9HGQAzjeCXla8D4JznG/t+3oOy8HxxEhrQHrZYWogKp2Ia2YDzbiFRmH9qADuwjSeSDw3SGMwr6Pjq2QWb1kiJY9k8lmWICL8EZJpA8fFouPrY7TV/vfZ0I2rVdnKw1k+sE+aUkZ+6SGGVRCN7mvOA4OAmjRSpkYcqDfcpdkBAwT/JjstIk6upsj7ox54ByEvIgSt5cLDowyOFzYONTtGkDOdtIAhRToIYQmYICq12OWu5SaUj3YkkTRvLI/gJSRMH83sEfiJHgcalMPZRRTKS7K0s5uvENtGa13/Wu1mvc8NXfd4cDvxOpN38aNuMjUv8C);strokeColor=none;spacingTop=-3;spacingBottom=-3;spacingLeft=-3;spacingRight=-3;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-794" vertex="1">
          <mxGeometry x="23" y="13" width="16" height="22" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-799" style="vsdxID=735;rotation=180;fillColor=#FFFFFF;gradientColor=none;shape=stencil(fVTtboMwDHwVlAdwkzifEvAu1UoHWtdOlG7t28/BoYXS7Z/lA99dfEl5brdfTXEe+tNH89PthrYS3bFt+m4Qdbk/9c17f7ocd3X5tR3auvw8fTfFtRLWgtSiuFVCgrRiU5dvlz5BqhKoIEEqY8VVV0JRidRMpQKM1MVKaHCOmqkKoDCNOXTHkUCOwzGCe9H2HrxZkkpm9PTDRAmomTFQaZgRwRpmDDrhs9HGQAzjeCXla8D4JznG/t+3oOy8HxxEhrQHrZYWogKp2Ia2YDzbiFRmH9qADuwjSeSDw3SGMwr6Pjq2QWb1kiJY9k8lmWICL8EZJpA8fFouPrY7TV/vfZ0I2rVdnKw1k+sE+aUkZ+6SGGVRCN7mvOA4OAmjRSpkYcqDfcpdkBAwT/JjstIk6upsj7ox54ByEvIgSt5cLDowyOFzYONTtGkDOdtIAhRToIYQmYICq12OWu5SaUj3YkkTRvLI/gJSRMH83sEfiJHgcalMPZRRTKS7K0s5uvENtGa13/Wu1mvc8NXfd4cDvxOpN38aNuMjUv8C);strokeColor=none;spacingTop=-3;spacingBottom=-3;spacingLeft=-3;spacingRight=-3;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-794" vertex="1">
          <mxGeometry x="18" y="19" width="16" height="22" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-800" style="vsdxID=736;rotation=240;fillColor=#FFFFFF;gradientColor=none;shape=stencil(fVTtboMwDHwVlAdwkzifEvAu1UoHWtdOlG7t28/BoYXS7Z/lA99dfEl5brdfTXEe+tNH89PthrYS3bFt+m4Qdbk/9c17f7ocd3X5tR3auvw8fTfFtRLWgtSiuFVCgrRiU5dvlz5BqhKoIEEqY8VVV0JRidRMpQKM1MVKaHCOmqkKoDCNOXTHkUCOwzGCe9H2HrxZkkpm9PTDRAmomTFQaZgRwRpmDDrhs9HGQAzjeCXla8D4JznG/t+3oOy8HxxEhrQHrZYWogKp2Ia2YDzbiFRmH9qADuwjSeSDw3SGMwr6Pjq2QWb1kiJY9k8lmWICL8EZJpA8fFouPrY7TV/vfZ0I2rVdnKw1k+sE+aUkZ+6SGGVRCN7mvOA4OAmjRSpkYcqDfcpdkBAwT/JjstIk6upsj7ox54ByEvIgSt5cLDowyOFzYONTtGkDOdtIAhRToIYQmYICq12OWu5SaUj3YkkTRvLI/gJSRMH83sEfiJHgcalMPZRRTKS7K0s5uvENtGa13/Wu1mvc8NXfd4cDvxOpN38aNuMjUv8C);strokeColor=none;spacingTop=-3;spacingBottom=-3;spacingLeft=-3;spacingRight=-3;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-794" vertex="1">
          <mxGeometry x="11" y="18" width="16" height="22" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-801" style="vsdxID=737;rotation=300;fillColor=#FFFFFF;gradientColor=none;shape=stencil(fVTtboMwDHwVlAdwkzifEvAu1UoHWtdOlG7t28/BoYXS7Z/lA99dfEl5brdfTXEe+tNH89PthrYS3bFt+m4Qdbk/9c17f7ocd3X5tR3auvw8fTfFtRLWgtSiuFVCgrRiU5dvlz5BqhKoIEEqY8VVV0JRidRMpQKM1MVKaHCOmqkKoDCNOXTHkUCOwzGCe9H2HrxZkkpm9PTDRAmomTFQaZgRwRpmDDrhs9HGQAzjeCXla8D4JznG/t+3oOy8HxxEhrQHrZYWogKp2Ia2YDzbiFRmH9qADuwjSeSDw3SGMwr6Pjq2QWb1kiJY9k8lmWICL8EZJpA8fFouPrY7TV/vfZ0I2rVdnKw1k+sE+aUkZ+6SGGVRCN7mvOA4OAmjRSpkYcqDfcpdkBAwT/JjstIk6upsj7ox54ByEvIgSt5cLDowyOFzYONTtGkDOdtIAhRToIYQmYICq12OWu5SaUj3YkkTRvLI/gJSRMH83sEfiJHgcalMPZRRTKS7K0s5uvENtGa13/Wu1mvc8NXfd4cDvxOpN38aNuMjUv8C);strokeColor=none;spacingTop=-3;spacingBottom=-3;spacingLeft=-3;spacingRight=-3;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="ZVaZIW3ceO06EkHoMhZQ-794" vertex="1">
          <mxGeometry x="8" y="11" width="16" height="22" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-312" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$M_1$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" vertex="1" parent="1">
          <mxGeometry x="-1568.16" y="257.25" width="100" height="40" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-313" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$M_2$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" vertex="1" parent="1">
          <mxGeometry x="-1497.5" y="257.25" width="100" height="40" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-318" value="" style="group" vertex="1" connectable="0" parent="1">
          <mxGeometry x="-1180" y="600" width="73.87000000000012" height="56.57999999999993" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-317" value="" style="rounded=0;whiteSpace=wrap;html=1;labelBackgroundColor=#FFF4FE;noLabel=1;labelBorderColor=default;fillColor=#FFF4FE;strokeColor=#000000;" vertex="1" parent="RbdjuNJBBSJslo0sPhe3-318">
          <mxGeometry y="3.3899999999999864" width="70" height="50" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-805" style="vsdxID=790;fillColor=#d8d8d8;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=default;rounded=0;html=1;whiteSpace=wrap;container=0;" parent="RbdjuNJBBSJslo0sPhe3-318" vertex="1">
          <mxGeometry x="6.121342281879379" y="8.609887640449415" width="12.751677852348994" height="12.780898876404496" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-806" style="vsdxID=791;fillColor=#f7cbac;gradientColor=none;shape=stencil(rZCxDsMgEEN/5XQ7Ch26Af9yai6ASkN00Ib+fUkiRV26dfSTbck2JdDCUKrkO69xrMFinANLrOjMlIW95Oc8OrNQDc488ouhWdQIb4tXjYMzJDeQtiuQg26Wiz5N0BS1WJTkSjXm2aLqMJF4Vj2tpkS+BxDKyryc8nf3H5qHY9AUUzrWb+x78LBf4z4=);strokeColor=#000000;labelBackgroundColor=default;rounded=0;html=1;whiteSpace=wrap;container=0;" parent="RbdjuNJBBSJslo0sPhe3-318" vertex="1">
          <mxGeometry x="6.121342281879379" y="35.19415730337073" width="12.751677852348994" height="12.780898876404496" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-807" style="vsdxID=792;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=default;rounded=0;exitX=0.52;exitY=1.04;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.52;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="RbdjuNJBBSJslo0sPhe3-318" source="ZVaZIW3ceO06EkHoMhZQ-805" target="ZVaZIW3ceO06EkHoMhZQ-806" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="12.752214765100689" y="21.902022471910072" as="sourcePoint" />
            <mxPoint x="12.752214765100689" y="35.19415730337073" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="12" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-810" value="&lt;span style=&quot;&quot;&gt;query&lt;/span&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;labelBackgroundColor=none;container=0;" parent="RbdjuNJBBSJslo0sPhe3-318" vertex="1">
          <mxGeometry x="18.87000000000012" y="26.579999999999927" width="50" height="30" as="geometry" />
        </mxCell>
        <mxCell id="ZVaZIW3ceO06EkHoMhZQ-811" value="anchor" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;labelBackgroundColor=none;container=0;" parent="RbdjuNJBBSJslo0sPhe3-318" vertex="1">
          <mxGeometry x="13.870000000000118" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-319" value="&lt;font style=&quot;font-size: 18px;&quot; face=&quot;Calibri&quot;&gt;&lt;b&gt;Ranking&lt;/b&gt;&lt;/font&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#FFF4FE;strokeColor=#9673a6;labelBorderColor=none;" vertex="1" parent="1">
          <mxGeometry x="-1085" y="607.38" width="82" height="35.82" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-322" style="vsdxID=802;edgeStyle=orthogonalEdgeStyle;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=1;exitY=0.5;exitDx=0;exitDy=0;entryX=0.746;entryY=1.004;entryDx=0;entryDy=0;entryPerimeter=0;" edge="1" parent="1" source="75" target="126">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="770" y="330" as="sourcePoint" />
            <mxPoint x="801" y="330" as="targetPoint" />
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-323" value="&lt;b style=&quot;border-color: var(--border-color); font-family: Calibri; font-size: 16px;&quot;&gt;Update \(\mathcal{T}^k\)&lt;br style=&quot;border-color: var(--border-color);&quot;&gt;based on&lt;br style=&quot;border-color: var(--border-color);&quot;&gt;ranking result&lt;/b&gt;" style="edgeLabel;html=1;align=left;verticalAlign=middle;resizable=0;points=[];" vertex="1" connectable="0" parent="RbdjuNJBBSJslo0sPhe3-322">
          <mxGeometry x="-0.3113" relative="1" as="geometry">
            <mxPoint x="-22" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="15" value="&lt;p style=&quot;align:center;margin-left:0;margin-right:0;margin-top:0px;margin-bottom:0px;text-indent:0;valign:middle;direction:ltr;&quot;&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;Masked &lt;/b&gt;&lt;/font&gt;&lt;font style=&quot;font-size:16px;font-family:Calibri;color:#000000;direction:ltr;letter-spacing:0px;line-height:120.00001%;opacity:1&quot;&gt;&lt;b&gt;Language Model&#xa;&lt;/b&gt;&lt;/font&gt;&lt;/p&gt;" style="verticalAlign=middle;align=center;vsdxID=183;fillColor=#bdd7ee;gradientColor=none;shape=stencil(rVLtjoMgEHwVsv9FMbWHCfIupKKS48Ss3NW+fRH7QXpNc8n1F8vsZmayO2Ie1KTJ7NF96qNp/dCAGQeNxoMUnUPdo/seWykm5QcpvtyPJksDjNZ7IKdQFAXkUlgzRrzmtNj9qaHwQDA0SlpUQDA0qpKWEMnDxDpZhWfJ1GLmDJ1X3rixgYBZhb3OAkHWWdVHaD5qPd2+iW7ClYgyyvkmuuOUbap3h2+QTclSN9e1vUDvHmt288g/osf37eXZVsrLHRhle/h15f+f4iEz+Rapzli75W/F0sjlMZzyDA==);strokeColor=#000000;labelBackgroundColor=none;rounded=0;html=1;whiteSpace=wrap;" parent="1" vertex="1">
          <mxGeometry x="400.5" y="516" width="472" height="18" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-326" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\mathcal{T}^{k}$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" vertex="1" parent="1">
          <mxGeometry x="322.5" y="144" width="180" height="40" as="geometry" />
        </mxCell>
        <mxCell id="RbdjuNJBBSJslo0sPhe3-327" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\mathcal{T}^{k}$$&lt;/font&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;" vertex="1" parent="1">
          <mxGeometry x="599" y="144" width="180" height="40" as="geometry" />
        </mxCell>
        <mxCell id="2" value="Connector" parent="0" />
        <mxCell id="218" style="vsdxID=823;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;entryX=0.5033557046979866;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="2" source="190" target="191" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="459" y="255" as="sourcePoint" />
            <mxPoint x="459" y="281" as="targetPoint" />
            <Array capacity="4" as="points">
              <mxPoint x="459" y="255" />
            </Array>
            <mxPoint x="12" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="223" parent="2" vertex="1">
          <mxGeometry x="660" y="369" as="geometry" />
        </mxCell>
        <mxCell id="229" style="vsdxID=802;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=5;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=1;exitY=0.4943820224719101;exitDx=0;exitDy=0;exitPerimeter=0;entryX=-0.005319148936170213;entryY=0.5056179775280899;entryDx=0;entryDy=0;entryPerimeter=0" parent="2" source="191" target="75" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="533" y="325" as="sourcePoint" />
            <mxPoint x="564" y="325" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="230" style="vsdxID=792;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.52;exitY=1.04;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.52;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="2" source="192" target="193" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="409" y="314" as="sourcePoint" />
            <mxPoint x="409" y="340" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="12" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="246" style="vsdxID=482;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=1;exitY=0.5042735042735043;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0;entryY=0.5042735042735043;entryDx=0;entryDy=0;entryPerimeter=0" parent="2" source="125" target="126" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="622" y="196" as="sourcePoint" />
            <mxPoint x="656" y="196" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="247" style="vsdxID=452;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.5384615384615384;exitY=1;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.5384615384615384;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="2" source="117" target="119" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="743" y="213" as="sourcePoint" />
            <mxPoint x="743" y="227" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-13" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="248" value="" style="vsdxID=450;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;align=center;exitX=0.46153846153846156;exitY=1;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.46153846153846156;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="2" source="116" target="118" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="698" y="213" as="sourcePoint" />
            <mxPoint x="698" y="227" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="12" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="249" style="vsdxID=446;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.8461538461538461;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.5384615384615384;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="2" source="115" target="117" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="725" y="182" as="sourcePoint" />
            <mxPoint x="743" y="200" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="4" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="250" style="vsdxID=445;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.15384615384615385;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.46153846153846156;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="2" source="115" target="116" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="716" y="182" as="sourcePoint" />
            <mxPoint x="698" y="200" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-4" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="251" style="vsdxID=427;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.5384615384615384;exitY=1;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.5384615384615384;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="2" source="109" target="112" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="469" y="213" as="sourcePoint" />
            <mxPoint x="469" y="227" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-13" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="252" style="vsdxID=426;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.8461538461538461;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.5384615384615384;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="2" source="108" target="111" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="429" y="211" as="sourcePoint" />
            <mxPoint x="438" y="227" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="8" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="253" value="" style="vsdxID=425;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;align=center;exitX=0.15384615384615385;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.46153846153846156;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="2" source="108" target="110" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="420" y="211" as="sourcePoint" />
            <mxPoint x="411" y="227" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-9" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="286" style="vsdxID=420;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.15384615384615385;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.46153846153846156;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="2" source="107" target="108" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="442" y="182" as="sourcePoint" />
            <mxPoint x="424" y="200" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="-4" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="287" style="vsdxID=421;edgeStyle=none;startArrow=none;endArrow=block;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;exitX=0.8461538461538461;exitY=0.8461538461538461;exitDx=0;exitDy=0;exitPerimeter=0;entryX=0.5384615384615384;entryY=0;entryDx=0;entryDy=0;entryPerimeter=0" parent="2" source="107" target="109" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="451" y="182" as="sourcePoint" />
            <mxPoint x="469" y="200" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="4" as="offset" />
          </mxGeometry>
        </mxCell>
        <mxCell id="219" parent="2" vertex="1">
          <mxGeometry x="660" y="410" as="geometry" />
        </mxCell>
        <mxCell id="221" parent="2" vertex="1">
          <mxGeometry x="660" y="410" as="geometry" />
        </mxCell>
        <mxCell id="225" parent="2" vertex="1">
          <mxGeometry x="660" y="418" as="geometry" />
        </mxCell>
        <mxCell id="226" style="vsdxID=819;edgeStyle=none;startArrow=none;endArrow=none;startSize=5;endSize=2;strokeColor=#000000;spacingTop=0;spacingBottom=0;spacingLeft=0;spacingRight=0;verticalAlign=middle;html=1;labelBackgroundColor=#ffffff;rounded=0;entryX=0.5037593984962406;entryY=1.0588235294117647;entryDx=0;entryDy=0;entryPerimeter=0" parent="2" source="225" target="50" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="660" y="418" as="sourcePoint" />
            <mxPoint x="660" y="403" as="targetPoint" />
            <Array capacity="4" as="points" />
            <mxPoint x="12" as="offset" />
          </mxGeometry>
        </mxCell>
      </root>
    </mxGraphModel>
  </diagram>
</mxfile>

